Theoretical and Experimental Evaluation of AoA Estimation in Single-Anchor 5G Uplink Positioning

As we move towards 6G, the demand for high-precision, cost-effective positioning solutions becomes increasingly critical. Single-anchor positioning offers a promising alternative to traditional multi-anchor approaches, particularly in complex propagation environments where infrastructure costs and deployment constraints present significant challenges. This paper provides a comprehensive evaluation of key algorithmic choices in the development of a single-anchor 5G uplink positioning testbed. Our developed testbed uses angle of arrival (AoA) estimation combined with range measurements from an ultra-wideband pair, to derive the position. The simulations conducted assess the impact of the selected algorithms on channel order and AoA estimation, while the influence of antenna calibration errors on AoA estimation is also examined. Finally, we compare simulations and results obtained from our developed platform.

==> COE/2P10.tex <==
-5 77	10	0
-4 88	36	0
-3 90	78	0
-2 86	99	0
-1 89	100	0
0 91	100	0
1 83	100	0
2 86	100	0
3 84	100	0
4 87	100	0
5 87	100	0
6 91	100	0
7 91	100	0
8 80	100	0
9 89	100	0
10 91	100	0

==> COE/2P15.tex <==
-5 93	100	0
-4 94	100	0
-3 87	100	0
-2 93	100	0
-1 87	100	0
0 96	100	0
1 88	100	0
2 91	100	0
3 87	100	0
4 95	100	10
5 94	100	77
6 85	100	100
7 89	100	100
8 95	100	100
9 89	100	100
10 92	100	100

==> COE/2P20.tex <==
-5	93	100	0
-4	90	100	0
-3	90	100	0
-2	84	100	0
-1	93	100	0
0	87	100	8
1	83	100	46
2	88	100	94
3	90	100	100
4	88	100	100
5	85	100	100
6	90	100	100
7	88	100	100
8	92	100	100
9	90	99	100
10	90	100	100

==> COE/2P5.tex <==
-5	16	0	0
-4	22	0	0
-3	30	0	0
-2	38	1	0
-1	50	1	0
0	83	11	0
1	89	32	0
2	95	59	0
3	82	96	0
4	84	100	0
5	90	100	0
6	92	100	0
7	85	100	0
8	89	100	0
9	87	100	0
10	93	100	0

==> COE/3P10.tex <==
-5	14	0	0
-4	10	0	0
-3	6	0	0
-2	6	0	0
-1	12	0	0
0	7	0	0
1	15	0	0
2	25	0	0
3	23	0	0
4	23	1	0
5	39	2	0
6	56	7	0
7	68	13	0
8	83	27	0
9	94	64	0
10	100	81	0

==> COE/3P15.tex <==
-5	16	0	0
-4	26	0	0
-3	26	1	0
-2	36	2	0
-1	51	4	0
0	71	9	0
1	82	22	0
2	94	43	0
3	100	79	0
4	100	95	0
5	100	99	0
6	100	100	0
7	100	100	0
8	100	100	0
9	100	100	0
10	100	100	0

==> COE/3P20.tex <==
-5	35	2	0
-4	71	10	0
-3	90	13	0
-2	97	44	0
-1	96	73	0
0	99	95	0
1	100	100	0
2	100	100	0
3	100	100	0
4	100	100	0
5	100	100	0
6	100	100	0
7	100	100	3
8	100	100	28
9	100	100	86
10	100	100	100

==> COE/3P5.tex <==
-5	5	0	0
-4	4	0	0
-3	6	0	0
-2	8	0	0
-1	13	0	0
0	6	0	0
1	8	0	0
2	12	0	0
3	15	0	0
4	11	0	0
5	11	0	0
6	11	0	0
7	9	0	0
8	7	0	0
9	15	0	0
10	14	0	0

==> COE/3_elements.tex <==
-5	3.90000000000000	0.800000000000000	0	0.100000000000000	0	0	0	0	0	0
-4	12.3000000000000	2.60000000000000	0.400000000000000	0	0	0	0	0	0	0
-3	31.4000000000000	5.10000000000000	0.600000000000000	0.100000000000000	0.100000000000000	0	0	0	0	0
-2	62.5000000000000	13.2000000000000	1.60000000000000	0	0	0	0	0	0	0
-1	91.6000000000000	34.3000000000000	3.70000000000000	0.100000000000000	0	0.800000000000000	0	0	0	0
0	99.1000000000000	64.7000000000000	9.80000000000000	0.500000000000000	0	12.2000000000000	0	0	0	0
1	100	93.1000000000000	22.7000000000000	0.200000000000000	0.200000000000000	64.5000000000000	1	0	0	0
2	100	99.9000000000000	52	1.90000000000000	0.100000000000000	98.8000000000000	16.2000000000000	0	0	0
3	100	100	84.4000000000000	6.70000000000000	0.100000000000000	100	74.4000000000000	0.300000000000000	0	0
4	100	100	98.1000000000000	15	0.200000000000000	100	99.8000000000000	4.50000000000000	0	0
5	100	100	99.9000000000000	34.5000000000000	0.300000000000000	100	100	43.2000000000000	0	0
6	100	100	100	68.9000000000000	0.600000000000000	100	100	95.5000000000000	0	0
7	100	100	100	92.9000000000000	1	100	100	100	2.10000000000000	0
8	100	100	100	100	2.20000000000000	100	100	100	20	0
9	100	100	100	100	5.30000000000000	100	100	100	76.3000000000000	0
10	100	100	100	100	14.8000000000000	100	100	100	99.6000000000000	0

==> Data/0los.tex <==
-5	0.412769333890005	0.412825037343550	0.326938140443700	0.141967527495685
-4	0.339171632068484	0.349498623892660	0.283605174463095	0.127847379254743
-3	0.295786879357417	0.282942137114004	0.242345755799093	0.112912256026622
-2	0.254339479829615	0.251346016480688	0.209515301686070	0.101975993028947
-1	0.212637139277219	0.216306458239502	0.184972461467105	0.0912799060996572
0	0.188216946633398	0.189374221082977	0.170006515841534	0.0793985018251652
1	0.163070852699063	0.161807324984690	0.150122903357730	0.0708275170476927
2	0.148079309830913	0.145836852005818	0.134297070490244	0.0638417823658334
3	0.124721990843634	0.123574579386778	0.119354296159472	0.0576937494582147
4	0.107475159920792	0.109358708876232	0.101796236367699	0.0521575533315054
5	0.0962032327939125	0.0921315128188544	0.0953740137079550	0.0466135661953816
6	0.0841188028920989	0.0855517084800135	0.0810046287188625	0.0408544027444424
7	0.0777825173159094	0.0764019451292216	0.0735217713297288	0.0355611472814195
8	0.0682491538409070	0.0683712126091389	0.0624577615175938	0.0328171942942645
9	0.0597485815731201	0.0580286742114056	0.0595995526287068	0.0279842713391125
10	0.0521167247627841	0.0525144727259501	0.0521528400933241	0.0254270420014914

==> Data/2despritextime.tex <==
2	0.00517253000000000
3	0.00619453000000000
4	0.00604314000000000
5	0.00693878000000000
6	0.00772074000000000
7	0.00868525000000000
8	0.00869393000000000
9	0.0100809900000000
10	0.0106987100000000
11	0.0118202100000000
12	0.0130888700000000
13	0.0137825500000000
14	0.0139023100000000
15	0.0157718500000000
16	0.0173496800000000
17	0.0171645000000000
18	0.0181679800000000
19	0.0196756500000000
20	0.0210569000000000
21	0.0220335700000000
22	0.0242987000000000
23	0.0245536500000000
24	0.0254537600000000
25	0.0273752300000000
26	0.0286052600000000
27	0.0290124100000000
28	0.0477429600000000
29	0.0506791100000000
30	0.0531460500000000
31	0.0560111600000000
32	0.0684996200000000
33	0.0777597000000000
34	0.0824369900000000
35	0.0810805600000000
36	0.0806869500000000
37	0.0838251100000000
38	0.0871831300000000
39	0.0885780600000000
40	0.0972895500000000
41	0.100534550000000
42	0.10914403300000000
43	0.10952789500000000
44	0.109222820000000
45	0.110632560000000
46	0.111990540000000
47	0.112860790000000
48	0.113435660000000
49	0.113064770000000
50	0.113558960000000
51	0.116116210000000
52	0.119037450000000
53	0.123928530000000
54	0.127046570000000
55	0.131166820000000
56	0.135090770000000
57	0.137730680000000
58	0.140244530000000
59	0.145081490000000
60	0.146279810000000

==> Data/2despritfinalres.tex <==
-5	0.888998487444455	0.778527808095951	0.721109865264223	0.683091656718262	0.688756311509750	0.650232891548660	0.674403008062989	0.667352472477449	0.660662261951893	0.644797942324629	0.676584057369206	0.668002498184245	0.632260288239185	0.706891395430303	0.651315296548518	0.647572325807104	0.652900903057369	0.644751330060113	0.672001060463657	0.660342710922124	0.682397212839488	0.594502567275220	0.678492671142106	0.666780189292073	0.644505599261539	0.650371534387423	0.684029327276585	0.667285440895515	0.659034529751416	0.637925087582919	0.658881138600379	0.667642251911245	0.654343733235762	0.681105699248663	0.646067904043390	0.649576314210993	0.674656545752970	0.631106633341289	0.660409992833063	0.674649514770424	0.665483273019839	0.668689089035455	0.677021269804047	0.680787409711985	0.676606607265650	0.669798242182043	0.624276747313872	0.640825364431770	0.647879180248164	0.667185486436020	0.656176259304019	0.677051351730296	0.669424007253910	0.685223254392619	0.650073905192068	0.653096827710971	0.650023559929773	0.626586031907524	0.676897093365253
-4	0.803428925739407	0.719926005464330	0.673110709214100	0.655230673873962	0.602122033586991	0.617091102223719	0.620135214017510	0.626106267327352	0.622166384109579	0.588408974160677	0.601435843414577	0.583628462574976	0.622776353972180	0.591446988693679	0.594777598226447	0.595868486338088	0.599503173485793	0.593959990608976	0.566367921484913	0.592752165302576	0.589316042033289	0.585476414438318	0.571657176011186	0.593762593541570	0.598813292889004	0.603251023267030	0.590530844080450	0.616587451318478	0.581199923872698	0.601728182142626	0.596216938550886	0.586694502552409	0.587356905605852	0.573730734419195	0.576695603980626	0.591203904572055	0.610595954227786	0.639671808663536	0.576368740919496	0.600403607705338	0.615485979047172	0.635486047951312	0.579656703913280	0.623233359078726	0.632682475482744	0.610998380600285	0.595268325733118	0.580061769090778	0.603757401574301	0.611906296714459	0.612690423488953	0.592810950109030	0.592852561088583	0.593695948858750	0.581277015285464	0.604248159169200	0.601987073453510	0.618067180738479	0.607642893862711
-3	0.822276143861748	0.672717182054843	0.670052064068883	0.634328501003969	0.642389442226328	0.573628955026167	0.518543093267888	0.584936125602664	0.533664860807601	0.561907727805169	0.559223940906766	0.557058572930375	0.539371125600958	0.548794530647256	0.549470880312210	0.509506900595644	0.542578136708134	0.529753185942048	0.538494264062063	0.544386650663429	0.539683637209769	0.546525546566920	0.545031221747673	0.544832910633480	0.526267638419659	0.515739730292492	0.508652131982345	0.549774648117546	0.557422873433411	0.535241976098414	0.550649850265785	0.539059171001875	0.500725390696043	0.539950461745252	0.555747968569436	0.549827850427354	0.551924749760386	0.541215127654779	0.560939895046015	0.491654160283102	0.526726474767016	0.539449768835756	0.539071776121988	0.526828698510295	0.529530855882207	0.566479704529497	0.508793752393064	0.522256113183704	0.541573103079921	0.506530611227701	0.545192681584772	0.513524497963126	0.518419516722408	0.517363226256344	0.546192365629283	0.543829230201967	0.514939863889952	0.541132846414981	0.554017064328777
-2	0.795141088135713	0.633421299481986	0.628426075934648	0.557319033452969	0.573862683933725	0.550586254637492	0.520979537562563	0.533566493542111	0.495187076417528	0.488972757433662	0.501691413374871	0.489499641416130	0.480364530906037	0.497764389821151	0.497541557640533	0.498061013510404	0.478645960365761	0.500250982692916	0.478631312007688	0.529975796935196	0.478354246181772	0.505118805069864	0.482486415816969	0.477916454885718	0.483356932536697	0.518471876998316	0.478959753303889	0.497856762423690	0.482762674541972	0.508483965319164	0.490466930947273	0.474009079981894	0.505176514514493	0.463227742612997	0.454025724176413	0.492230465132633	0.490800857528882	0.485219618831899	0.489227312214798	0.506593181737761	0.489448429680953	0.492173138247449	0.477340779091898	0.471212824142313	0.499454975391830	0.532796907306087	0.468047571423460	0.447794665034438	0.458568277112269	0.480057325823617	0.479645881670933	0.476983854155727	0.467536414032447	0.453293439817780	0.494511264329280	0.463579850134394	0.484848155364973	0.478937508162846	0.511492551376021
-1	0.773096502515003	0.660344266925369	0.579915945091127	0.551573683735525	0.538980375324280	0.469690571908957	0.498237337278599	0.496838754032143	0.465145932322720	0.488872566954452	0.462613029919006	0.468619166927205	0.460612341227301	0.466057865803121	0.436642325892953	0.432207040623809	0.456628174984295	0.457620838553201	0.418695025236496	0.440845043061759	0.456028803441377	0.445750925532635	0.444197470014532	0.447162152395632	0.458424405767874	0.450436753835608	0.425343820285439	0.411953643024467	0.446300223804641	0.427266003784021	0.430212494944341	0.439628115740614	0.454534475824903	0.432052014332269	0.447650215080967	0.432741576360589	0.445201727991366	0.449548282930041	0.427373722613847	0.430976819698101	0.441203647399026	0.450480636528052	0.433368134266776	0.423069232141105	0.443216776935273	0.435839250219812	0.433383022555201	0.429423328959217	0.423256388094774	0.426336656272849	0.446339250273646	0.422841658114406	0.440526406148375	0.443711253422175	0.441645712740862	0.449317519651612	0.439009606211657	0.422044871247182	0.445539130360607
0	0.760738121804735	0.589993691599258	0.572326973490096	0.559013593858173	0.487687443130500	0.480008251486439	0.459404023422962	0.426964561282138	0.443227422546598	0.461481434127616	0.423571298017603	0.435334198465959	0.397932664232495	0.431594000264714	0.423356435767689	0.453966402197889	0.419131216772071	0.425519804908859	0.412697771657116	0.423228373913042	0.408521542363030	0.406733099377801	0.431591113592841	0.441399033177028	0.399354413912662	0.403785806840294	0.398001781916191	0.406346484859112	0.403107208050880	0.420599710444983	0.410773368211613	0.409332047232340	0.405118741694874	0.407643460973005	0.419165719773765	0.405849130059562	0.406949098413624	0.402357818377377	0.404617426499779	0.409450700595841	0.380562657484404	0.372059356996052	0.403725565665160	0.403805698424045	0.386392230361593	0.386056703925209	0.398487677277384	0.385914110131803	0.402221085753946	0.396926967421578	0.396024465405038	0.417619719871893	0.403826970270138	0.372915706946156	0.409824777144968	0.403045090496930	0.401287259039474	0.390999503088556	0.418996743263617
1	0.752976634804653	0.614663184850618	0.533803631612326	0.516463201805680	0.497228691715001	0.449147896204890	0.407642577624991	0.463288218985485	0.419862791296946	0.416188157435709	0.394151484894363	0.412894557570700	0.394822929243979	0.393480166054361	0.415875767860447	0.393505050830516	0.356900733550818	0.403299268890690	0.384344617556783	0.370267288720118	0.406295210634785	0.403186578430551	0.369511984061792	0.394322323622223	0.384209893922546	0.392552570928947	0.368197494971344	0.369783660188111	0.370896648090130	0.372384875009693	0.361339879899969	0.358122614261770	0.362605089067190	0.360133221492029	0.356327544202288	0.373915776219865	0.372865743819177	0.365576503606522	0.390087098009025	0.346853048400056	0.366837634584843	0.345241415637301	0.357031809682740	0.339768748906153	0.354827613652622	0.348589902230215	0.356546777131440	0.352689234732459	0.343221694272552	0.358670378837337	0.358584838220833	0.360013114477672	0.341944841578447	0.364034178385674	0.356614206551609	0.340349640522538	0.361930170038201	0.354409775264522	0.371099712900180
2	0.720971323162683	0.557244549258845	0.514358787614634	0.474466986018354	0.493095376245906	0.443675031531182	0.430715035698894	0.406058970684521	0.390464493404905	0.410247323019191	0.405200314118650	0.369108526843961	0.379091573134851	0.392448509637165	0.358515125108356	0.367884899970412	0.371917597331439	0.368790814592176	0.355400365743551	0.338688509640368	0.365888305530809	0.340230860509242	0.365541779015846	0.331985298720079	0.356368107997445	0.343904228020413	0.355482434069771	0.338036489770453	0.352530876051140	0.351451806441585	0.333069621144557	0.355767030182091	0.346758842009478	0.343244188320748	0.344999903742562	0.325575073215370	0.344002851438399	0.339064336313045	0.329674468091475	0.344404371985680	0.350642747854462	0.340606042397172	0.348936649512162	0.322486440979197	0.341240046126239	0.334779250426673	0.325762880370939	0.315404769243306	0.322313560210283	0.326134028623193	0.337437083028546	0.323801640272613	0.326173561326222	0.331529345555080	0.332923917742642	0.329326164788765	0.322321771604358	0.312225531426620	0.323705641414149
3	0.737720054575253	0.540905639938933	0.488629049141310	0.451395702421745	0.409809847956788	0.398153142022491	0.384738408650032	0.364331286801295	0.376693449809526	0.389690218548772	0.401814833676667	0.352632428317661	0.382949733202050	0.346576389660096	0.334380895809968	0.356041609756358	0.339329326080094	0.341298280198455	0.337182015074631	0.332613632459831	0.341698498190586	0.352980173724427	0.338380209209619	0.339840661071483	0.333176738030977	0.363224367461470	0.324798936126085	0.333472688743697	0.315218302763385	0.327119627965486	0.336259126774032	0.354942872181792	0.326634398745846	0.321204261215685	0.313403596350885	0.319354194249456	0.326572720767960	0.316050857772518	0.289649032160196	0.318821373280196	0.312508251267060	0.307781103417774	0.319518811370904	0.316656017933203	0.299692195085184	0.303373801410312	0.306837092740885	0.300956498145308	0.297826977196527	0.292968396329355	0.307883848825602	0.300529300118441	0.306005493172670	0.293918073257614	0.301892903272989	0.310533703245029	0.293070497243654	0.304028314470841	0.289522117545506
4	0.735773329459620	0.527947539181357	0.480768952230851	0.437965161900881	0.414753814138714	0.407725478423653	0.385470128720031	0.360141623984519	0.363151795697186	0.359312789900604	0.333611523308131	0.366405785278977	0.372570794581380	0.329903311539162	0.331052683992762	0.331108902374959	0.333877488592947	0.310341372314746	0.318938766862339	0.321759515582759	0.320399256532236	0.320059437306023	0.289609640464365	0.299002234555968	0.325087766989688	0.316507923345354	0.302291079589533	0.304447066801965	0.299802897708865	0.290622279309942	0.295996829817129	0.291563253812422	0.290873221712570	0.300574774627198	0.284629453417730	0.297205239676715	0.302137229719515	0.287137683224894	0.293250232239793	0.282077128351367	0.273676587466041	0.292199883309300	0.289006653035446	0.288184431255302	0.276930059790882	0.280615022962370	0.304632822904663	0.281658079213808	0.288360745119388	0.258959651260257	0.282143832733634	0.277035187666739	0.273374075917625	0.265877128105725	0.262908266506392	0.271847495640715	0.276708711876533	0.274278079767323	0.258296664195187
5	0.736504537325095	0.533439419440686	0.466491105968868	0.433272618171716	0.410856648212672	0.392130085642983	0.380075915012063	0.369093247298221	0.321477471293258	0.333238001361623	0.318035435600917	0.318586484157754	0.334231840576384	0.362011942202314	0.317148221338044	0.318469597985367	0.313028321306743	0.318578165212511	0.301122919432468	0.293862621945220	0.280102486117474	0.316896676902995	0.292415595000011	0.307920800509910	0.294924967283192	0.282214670452878	0.288632521156421	0.309181814022882	0.287734360395240	0.285816441178962	0.280019800103233	0.282766347176263	0.264158820185358	0.280266580243710	0.282654072292578	0.274085858785949	0.272967428376273	0.282722483907298	0.280541504509873	0.278187909380445	0.251720806675668	0.262596417911794	0.279051528234563	0.261810646608735	0.249374626771117	0.256927419267381	0.252586649871255	0.259402929467915	0.259001001059597	0.251394515534953	0.245218535303857	0.265118602380329	0.268719419187528	0.260568105396587	0.240511869622231	0.267963767404138	0.258037140595211	0.252032675731015	0.237771931472016
6	0.737867655972614	0.528162279183021	0.453865958099390	0.421125349878732	0.387652838878152	0.387234382070662	0.351066308915199	0.333206047098934	0.356863862593589	0.327381330538463	0.313419061912868	0.300018707936325	0.318524690967710	0.309897366768104	0.307084142505379	0.303136164568101	0.300442067735154	0.294292210947762	0.290155681779497	0.283782181085405	0.295923353870139	0.271089803241096	0.287081907373255	0.284415750153631	0.275219432369833	0.281291668978399	0.265320209256878	0.273354843533089	0.280924592269075	0.294541075856830	0.275837448783807	0.270589591081257	0.273944386461605	0.270361077905976	0.269530625205476	0.255909085937695	0.287005579267920	0.274079184249238	0.255895358136254	0.262528611779234	0.246783661860998	0.271825534760992	0.253440448492576	0.259229351995521	0.256993812324041	0.239853600355257	0.241371060871221	0.245978786634168	0.226320178881381	0.262609833742568	0.245570663096184	0.227843488450004	0.235112579550230	0.239966586179885	0.242389854120901	0.249588012240771	0.228922473517272	0.236488773775468	0.224036402081798
7	0.702800722489053	0.510408452991274	0.461592890668178	0.411941637361641	0.395112334219380	0.369935296389794	0.357977576058457	0.335501968627777	0.330915340964231	0.313321796645729	0.306530897212638	0.319175603813480	0.293992700433454	0.306015856651074	0.302144634020547	0.286986907049445	0.283269175258205	0.287506600368138	0.279856905593866	0.293696310278171	0.277857686532270	0.275743568301608	0.280298883663734	0.279496432525527	0.283082206809816	0.268562628862760	0.265406749526587	0.240943338675793	0.262418679950076	0.261816538531427	0.262266149849818	0.241351016907566	0.267112192404806	0.248792510217340	0.264955559603124	0.263901088051358	0.245423574016795	0.248354654240713	0.249655791703353	0.242103035508157	0.234556367267967	0.235381435964523	0.243848809187948	0.222157682599481	0.232326369368085	0.225965781137363	0.223617523417301	0.226159400299530	0.235053689653979	0.214441034609463	0.226006841551442	0.226993119588963	0.209571133701271	0.238417695632344	0.225741010708315	0.215078482586362	0.223437855185143	0.227326418187037	0.223351403465174
8	0.708414199972275	0.523266088967593	0.459477354701348	0.399764948286801	0.376177600873103	0.343815884066367	0.333359305915960	0.324915143309831	0.313107516121169	0.305112696136307	0.306410686459077	0.298774653735869	0.298179525212222	0.284504793132878	0.285191591514126	0.273693473276929	0.274873204394973	0.276530162150913	0.278559600863890	0.269353377444001	0.263433452839223	0.261895961255283	0.254803198274012	0.277331544048953	0.254391847513815	0.244044259351328	0.269840673327248	0.272988755337267	0.249689266525914	0.252307069367312	0.259843869091864	0.236231741726520	0.234740449848623	0.242542359955314	0.234913581268429	0.265689433118099	0.236914013415643	0.236356800495772	0.231737991419996	0.224012485269718	0.226029927673460	0.229055970565607	0.226881891885092	0.229985818757496	0.222661070435180	0.228835161854784	0.211509272406536	0.211082687996497	0.208992904829375	0.211081672114040	0.207750905115593	0.210839180312152	0.221994264743987	0.209463991831035	0.203268043658642	0.203710156717948	0.204993001054638	0.210554877475189	0.205084184125659
9	0.696299571139374	0.528965692975378	0.438417085494513	0.411963284513297	0.373325561638422	0.349785544436343	0.330772762326160	0.329482052623246	0.313165757773480	0.290881257087204	0.293644614718964	0.299346483643763	0.286124913755359	0.277335164432429	0.273688350528482	0.303347827899038	0.289424670416147	0.264519431171373	0.256964574352291	0.253241843101433	0.267351517628535	0.271486816733183	0.253989330675887	0.249059068210345	0.248082530488590	0.268121479127837	0.246485427733976	0.249674495865163	0.243884414331702	0.231363187650567	0.251701951514646	0.239433035702180	0.237780718314423	0.237443188277927	0.244289355493263	0.231270614123879	0.232859842927699	0.216401864180500	0.215673992226559	0.227477611708797	0.217822862149090	0.221420336841539	0.212506401850657	0.215595715593211	0.202914319459097	0.208503131061067	0.212250773630318	0.227106036028018	0.212009350569725	0.208031932470771	0.203026394286164	0.209193393107342	0.205697179459489	0.201681149629607	0.192784721886044	0.218292201440715	0.197757338550713	0.199760363929236	0.200806548187703
10	0.690719810207627	0.508572129513991	0.442039356685027	0.399290487456104	0.384963939071597	0.353383365348060	0.332297542512216	0.310393936059990	0.317292784852365	0.299297067516529	0.294973297240535	0.289709481600577	0.276512727034928	0.283834287684344	0.269174548143790	0.250322298234414	0.266710965912427	0.258409734088814	0.259956139789056	0.257958448598002	0.250764572622914	0.262595771699585	0.241021009296848	0.249823069524140	0.246346375845834	0.240862690709103	0.240631728504172	0.237876438656476	0.237917886565194	0.231156277231059	0.234814208201769	0.232633981845382	0.226017812340727	0.234359219901779	0.240975066029124	0.210928412666283	0.229981050188441	0.208202697561310	0.205485466534197	0.210651585968997	0.238919748169121	0.193023250725573	0.200091422702795	0.219414656637493	0.200310777372233	0.205561601181126	0.197095490122142	0.209239021208088	0.199260052464996	0.197245400935224	0.188259420110509	0.202751847668718	0.197679022429750	0.188018769866655	0.185520911797193	0.193175446651607	0.191741250015889	0.189551945548688	0.193495778857142

==> Data/2esprit.tex <==
-5	0.888998487444455	0.778527808095951	0.721109865264223	0.683091656718262	0.688756311509750	0.650232891548660	0.674403008062989	0.667352472477449	0.660662261951893
-4	0.803428925739407	0.719926005464330	0.673110709214100	0.655230673873962	0.602122033586991	0.617091102223719	0.620135214017510	0.626106267327352	0.622166384109579
-3	0.822276143861748	0.672717182054843	0.670052064068883	0.634328501003969	0.642389442226328	0.573628955026167	0.518543093267888	0.584936125602664	0.533664860807601
-2	0.795141088135713	0.633421299481986	0.628426075934648	0.557319033452969	0.573862683933725	0.550586254637492	0.520979537562563	0.533566493542111	0.495187076417528
-1	0.773096502515003	0.660344266925369	0.579915945091127	0.551573683735525	0.538980375324280	0.469690571908957	0.498237337278599	0.496838754032143	0.465145932322720
0	0.760738121804735	0.589993691599258	0.572326973490096	0.559013593858173	0.487687443130500	0.480008251486439	0.459404023422962	0.426964561282138	0.443227422546598
1	0.752976634804653	0.614663184850618	0.533803631612326	0.516463201805680	0.497228691715001	0.449147896204890	0.407642577624991	0.463288218985485	0.419862791296946
2	0.720971323162683	0.557244549258845	0.514358787614634	0.474466986018354	0.493095376245906	0.443675031531182	0.430715035698894	0.406058970684521	0.390464493404905
3	0.737720054575253	0.540905639938933	0.488629049141310	0.451395702421745	0.409809847956788	0.398153142022491	0.384738408650032	0.364331286801295	0.376693449809526
4	0.735773329459620	0.527947539181357	0.480768952230851	0.437965161900881	0.414753814138714	0.407725478423653	0.385470128720031	0.360141623984519	0.363151795697186
5	0.736504537325095	0.533439419440686	0.466491105968868	0.433272618171716	0.410856648212672	0.392130085642983	0.380075915012063	0.369093247298221	0.321477471293258
6	0.737867655972614	0.528162279183021	0.453865958099390	0.421125349878732	0.387652838878152	0.387234382070662	0.351066308915199	0.333206047098934	0.356863862593589
7	0.702800722489053	0.510408452991274	0.461592890668178	0.411941637361641	0.395112334219380	0.369935296389794	0.357977576058457	0.335501968627777	0.330915340964231
8	0.708414199972275	0.523266088967593	0.459477354701348	0.399764948286801	0.376177600873103	0.343815884066367	0.333359305915960	0.324915143309831	0.313107516121169
9	0.696299571139374	0.528965692975378	0.438417085494513	0.411963284513297	0.373325561638422	0.349785544436343	0.330772762326160	0.329482052623246	0.313165757773480
10	0.690719810207627	0.508572129513991	0.442039356685027	0.399290487456104	0.384963939071597	0.353383365348060	0.332297542512216	0.310393936059990	0.317292784852365

==> Data/antenna_err.tex <==
-5	2.01477286685125	1.94473866914800	2.03286609517494	0.511812528178041	0.503016364495267	0.431412934715505	1.54518564515724	1.51629908038575	1.52428861378757
-4	2.01105845041858	1.95670483813047	2.02356797180191	0.444348563629949	0.438224851990790	0.415224149091196	1.51947650491871	1.49329384497732	1.52348577798927
-3	1.97249178604120	1.92876948647127	1.90012668076685	0.427280125912730	0.410578503896415	0.379328519783384	1.53074766764480	1.48751794650761	1.50236213928067
-2	1.93665150401408	1.96259977746930	1.96880608440043	0.382765381140979	0.399491545775911	0.341585303610657	1.49995878110033	1.49202266858102	1.48650395527226
-1	1.99198734985943	2.02816808988815	1.96938966566144	0.350721174154055	0.359231791979972	0.354100201696761	1.52867901372394	1.55385611199662	1.49383274887575
0	1.96964446918727	1.92475048482701	1.96108399924600	0.343334871517589	0.338246546537691	0.343979459493773	1.57370765010532	1.48654863379818	1.46596760082948
1	2.00383144176350	1.93797556220446	1.93317093706018	0.326975970065078	0.332788870054792	0.324040122376354	1.55855357367015	1.49028624299325	1.51353309274922
2	2.00041905259873	1.97174536488908	1.99342917558805	0.321520498568908	0.328436194040130	0.312839324493611	1.49334596460432	1.51716729529230	1.50471529544959
3	1.92193520364241	1.97314878629057	1.93814052234036	0.325114887385981	0.316648263051106	0.306953547390567	1.51398585264196	1.53979728579331	1.50310952173146
4	1.98689714630627	1.97131805660411	1.95561534697321	0.309870335785792	0.305694677206739	0.291507557690426	1.49745476158714	1.47926741194070	1.46655245063944
5	1.96655069321897	1.97419351600522	1.92962675979773	0.299259579629457	0.299386665835583	0.304400710225673	1.51304614404188	1.51275827228739	1.45516227013232
6	1.93745617731086	1.89252302484111	1.88847158296338	0.282810689331219	0.297911614217978	0.286289613041830	1.48165171818481	1.47596482834182	1.46051302282111
7	1.97638690695926	1.99721851271487	1.97316718036155	0.297679740660998	0.281591191092392	0.296065696285115	1.48283175579699	1.47611422816711	1.47018626513829
8	2.01159822056990	1.96148636939956	1.91767051213295	0.287736785969398	0.294630755417157	0.295671921240412	1.49853018788411	1.45927447567685	1.44938022758778
9	1.96952002553922	1.94864290480353	1.92416691816977	0.288585420629662	0.297250854034516	0.291449124424122	1.57774506590894	1.51287247531707	1.49931614872572
10	1.90660881068981	1.98358522314189	2.01410948932400	0.290427648477205	0.289433020708773	0.295878922885492	1.50663717928372	1.49677024310696	1.47529360912520

==> Data/cdfs/15m_2desprit.tex <==
0	0.00882814690755306
0.0125000000000000	0.00882814690755306
0.0249999999999999	0.0173514494329170
0.0374999999999999	0.0701743441194497
0.0499999999999998	0.0903122653115222
0.0624999999999999	0.0923542663587230
0.0749999999999998	0.0946927285190187
0.0874999999999998	0.111957618749536
0.0999999999999999	0.116170241549362
0.112500000000000	0.125251400369511
0.125000000000000	0.173141126779755
0.137500000000000	0.203398721074568
0.150000000000000	0.204723800947581
0.162500000000000	0.213186909726134
0.175000000000000	0.238124471067589
0.187500000000000	0.248203066607281
0.200000000000000	0.257797795541727
0.212500000000000	0.272238066949407
0.225000000000000	0.275011278807777
0.237500000000000	0.279033064880827
0.250000000000000	0.296618763824755
0.262500000000000	0.314579788937948
0.275000000000000	0.316472953455095
0.287500000000000	0.319113432436410
0.300000000000000	0.320850784731072
0.312500000000000	0.327510718071559
0.325000000000000	0.332154781734780
0.337500000000000	0.333187377539175
0.350000000000000	0.333914791104194
0.362500000000000	0.335156202918840
0.375000000000000	0.338662857642352
0.387500000000000	0.347584790786024
0.400000000000000	0.349066127611547
0.412500000000000	0.349752952362325
0.425000000000000	0.365092183784310
0.437500000000000	0.369122257025348
0.450000000000000	0.380420941314642
0.462500000000000	0.395055953212876
0.475000000000000	0.395950874634260
0.487500000000000	0.398253674695040
0.500000000000000	0.405144499578484
0.512500000000000	0.408434049506953
0.525000000000000	0.413429937625065
0.537500000000000	0.413738740611538
0.550000000000000	0.414619572728202
0.562500000000000	0.422806254229928
0.575000000000000	0.426501816577742
0.587500000000000	0.426978422719192
0.600000000000000	0.429816344063765
0.612500000000000	0.435332609737782
0.625000000000000	0.475030315455840
0.637500000000000	0.475832828740898
0.650000000000000	0.478757247661224
0.662500000000000	0.482803424406822
0.675000000000000	0.483087863089054
0.687500000000000	0.490257954132213
0.700000000000000	0.498237229525332
0.712500000000000	0.513798865682586
0.725000000000000	0.522053580189122
0.737500000000000	0.528920530967022
0.750000000000000	0.532301016207248
0.762500000000000	0.532310958505830
0.775000000000000	0.536184514870704
0.787500000000000	0.550314134498542
0.800000000000000	0.551937021894638
0.812500000000000	0.562172232372947
0.825000000000000	0.562977442582494
0.837500000000000	0.589079134388514
0.850000000000000	0.589279773593410
0.862500000000000	0.606843330618138
0.875000000000000	0.636859541604748
0.887500000000000	0.720824848543645
0.900000000000000	0.751416759620127
0.912500000000000	0.794465643360891
0.925000000000000	0.800545283155272
0.937500000000000	0.879574905941431
0.950000000000000	0.886218669664113
0.962500000000000	0.901188064676355
0.975000000000000	0.943092292425773
0.987500000000000	1.05482099890778
1	1.12166560442352

==> Data/cdfs/15m_esprit.tex <==
0	0.998218134418824
0.0125000000000000	0.998218134418824
0.0249999999999999	1.01006904839976
0.0374999999999999	1.01669034490398
0.0499999999999998	1.02278153148013
0.0624999999999999	1.03943567622220
0.0749999999999998	1.04620382455751
0.0874999999999998	1.07185689693694
0.0999999999999999	1.10095632730110
0.112500000000000	1.10579204205884
0.125000000000000	1.11524988272177
0.137500000000000	1.11561427290737
0.150000000000000	1.12061249847936
0.162500000000000	1.12808469451007
0.175000000000000	1.13330827457444
0.187500000000000	1.13815720701791
0.200000000000000	1.13906701365557
0.212500000000000	1.14119710837800
0.225000000000000	1.14476836475236
0.237500000000000	1.14834887914542
0.250000000000000	1.15315734363218
0.262500000000000	1.15734668343286
0.275000000000000	1.16290203956682
0.287500000000000	1.16409417087665
0.300000000000000	1.16483584262037
0.312500000000000	1.16488195375566
0.325000000000000	1.17021172635563
0.337500000000000	1.17269521818719
0.350000000000000	1.17933790321378
0.362500000000000	1.19388784257747
0.375000000000000	1.19602482791397
0.387500000000000	1.20055752081248
0.400000000000000	1.20172808237705
0.412500000000000	1.21022723362472
0.425000000000000	1.22243624307179
0.437500000000000	1.22246378829102
0.450000000000000	1.22709657232275
0.462500000000000	1.23149462943838
0.475000000000000	1.23392794938995
0.487500000000000	1.23740629560999
0.500000000000000	1.23800303983381
0.512500000000000	1.24852538894820
0.525000000000000	1.25522315862126
0.537500000000000	1.25547177490045
0.550000000000000	1.25716601197090
0.562500000000000	1.25846222809465
0.575000000000000	1.25886711707377
0.587500000000000	1.28025314183806
0.600000000000000	1.28444344283582
0.612500000000000	1.28563299382057
0.625000000000000	1.31385022094629
0.637500000000000	1.31475449552195
0.650000000000000	1.32701833701642
0.662500000000000	1.33112345840064
0.675000000000000	1.33692571085930
0.687500000000000	1.34092688859100
0.700000000000000	1.34315070050823
0.712500000000000	1.34713727763771
0.725000000000000	1.35330715661786
0.737500000000000	1.35888598793572
0.750000000000000	1.36988706318064
0.762500000000000	1.38735160544191
0.775000000000000	1.38834946988009
0.787500000000000	1.39105404742129
0.800000000000000	1.39424721998348
0.812500000000000	1.39500533193983
0.825000000000000	1.40746916897199
0.837500000000000	1.41343028851332
0.850000000000000	1.42089861070247
0.862500000000000	1.42191571519607
0.875000000000000	1.42814119633481
0.887500000000000	1.45381638301717
0.900000000000000	1.45796308663973
0.912500000000000	1.47858901976160
0.925000000000000	1.49432321125450
0.937500000000000	1.49751163901413
0.950000000000000	1.60431321938328
0.962500000000000	1.62150222917589
0.975000000000000	1.66936669798632
0.987500000000000	1.70758968342809
1	1.90782670116149

==> Data/cdfs/15m_music.tex <==
0	1.01000000000000
0.0125000000000000	1.01000000000000
0.0249999999999999	1.01555555555556
0.0374999999999999	1.02400000000000
0.0499999999999998	1.02625000000000
0.0624999999999999	1.03818181818182
0.0749999999999998	1.04545454545454
0.0874999999999998	1.07363636363636
0.0999999999999999	1.07500000000000
0.112500000000000	1.09727272727273
0.125000000000000	1.10090909090909
0.137500000000000	1.11600000000000
0.150000000000000	1.12090909090909
0.162500000000000	1.12818181818182
0.175000000000000	1.13363636363636
0.187500000000000	1.13700000000000
0.200000000000000	1.13727272727272
0.212500000000000	1.14181818181818
0.225000000000000	1.15333333333333
0.237500000000000	1.15800000000000
0.250000000000000	1.16200000000000
0.275000000000000	1.16500000000000
0.287500000000000	1.16545454545454
0.300000000000000	1.16555555555556
0.312500000000000	1.16888888888889
0.325000000000000	1.17090909090909
0.337500000000000	1.17285714285714
0.350000000000000	1.18090909090909
0.362500000000000	1.19636363636364
0.375000000000000	1.20000000000000
0.387500000000000	1.20090909090909
0.400000000000000	1.20750000000000
0.412500000000000	1.20909090909091
0.425000000000000	1.21428571428572
0.437500000000000	1.22181818181818
0.450000000000000	1.23000000000000
0.462500000000000	1.23363636363636
0.475000000000000	1.23400000000000
0.487500000000000	1.23818181818182
0.500000000000000	1.23909090909091
0.512500000000000	1.24727272727273
0.525000000000000	1.25545454545454
0.537500000000000	1.25636363636364
0.550000000000000	1.25800000000000
0.562500000000000	1.25909090909091
0.575000000000000	1.27800000000000
0.587500000000000	1.28200000000000
0.600000000000000	1.28363636363636
0.612500000000000	1.28545454545455
0.625000000000000	1.31400000000000
0.637500000000000	1.31545454545454
0.650000000000000	1.32727272727273
0.662500000000000	1.33222222222222
0.675000000000000	1.33454545454546
0.687500000000000	1.33700000000000
0.700000000000000	1.33909090909091
0.712500000000000	1.34727272727273
0.725000000000000	1.35272727272727
0.737500000000000	1.35909090909091
0.750000000000000	1.37000000000000
0.762500000000000	1.38600000000000
0.775000000000000	1.38818181818182
0.787500000000000	1.39000000000000
0.800000000000000	1.39363636363636
0.812500000000000	1.39363636363637
0.825000000000000	1.41400000000000
0.837500000000000	1.42090909090909
0.850000000000000	1.42272727272727
0.862500000000000	1.42636363636364
0.875000000000000	1.44727272727273
0.887500000000000	1.45272727272727
0.900000000000000	1.45818181818182
0.912500000000000	1.47818181818182
0.925000000000000	1.49363636363636
0.937500000000000	1.49800000000000
0.950000000000000	1.60363636363636
0.962500000000000	1.62272727272727
0.975000000000000	1.66727272727273
0.987500000000000	1.70818181818182
1	1.90800000000000

==> Data/cdfs/50m_2desprit.tex <==
0	3.48441855056768
0.0125000000000000	3.48441855056768
0.0249999999999999	3.53601865274128
0.0374999999999999	3.55494627094893
0.0499999999999998	3.56152655061659
0.0624999999999999	3.60325940069063
0.0749999999999998	3.66494482562497
0.0874999999999998	3.66749987501031
0.0999999999999999	3.67936490493416
0.112500000000000	3.68285378244185
0.125000000000000	3.70834801274957
0.137500000000000	3.72109075567052
0.150000000000000	3.73444850425620
0.162500000000000	3.74133953943932
0.175000000000000	3.74876002725482
0.187500000000000	3.76258593229942
0.200000000000000	3.76781913221341
0.212500000000000	3.77618374112068
0.225000000000000	3.78545529999951
0.237500000000000	3.78981591102129
0.250000000000000	3.78995937090111
0.262500000000000	3.79685448901720
0.275000000000000	3.80654867505986
0.287500000000000	3.85238249285174
0.300000000000000	3.85774561055024
0.312500000000000	3.86412526003144
0.325000000000000	3.86841221503547
0.337500000000000	3.87139036624435
0.350000000000000	3.87292726280269
0.362500000000000	3.87307613485699
0.375000000000000	3.87310315850133
0.387500000000000	3.87351573239003
0.400000000000000	3.88393083588726
0.412500000000000	3.88987815156188
0.425000000000000	3.89440386048161
0.437500000000000	3.89606015520538
0.450000000000000	3.90088289759810
0.462500000000000	3.90767596437161
0.475000000000000	3.91576456656673
0.487500000000000	3.91696397486300
0.500000000000000	3.94573223522007
0.512500000000000	3.94722347761811
0.525000000000000	3.94849715261309
0.537500000000000	3.96379425179844
0.550000000000000	3.96917805563014
0.562500000000000	3.98697002993921
0.575000000000000	3.99647128397882
0.587500000000000	3.99919433756670
0.600000000000000	4.00386886082651
0.612500000000000	4.00484684370648
0.625000000000000	4.01910351454330
0.637500000000000	4.01913054395638
0.650000000000000	4.03386096295606
0.662500000000000	4.04131552460727
0.675000000000000	4.04766709880514
0.687500000000000	4.05453949550687
0.700000000000000	4.07892711664446
0.712500000000000	4.08152050400862
0.725000000000000	4.08922043246139
0.737500000000000	4.09292747148530
0.750000000000000	4.09540655966228
0.762500000000000	4.10552175921205
0.775000000000000	4.11883056557276
0.787500000000000	4.12358117181888
0.800000000000000	4.12816329716527
0.812500000000000	4.21579151642234
0.825000000000000	4.22632925936511
0.837500000000000	4.35563951610627
0.850000000000000	4.37256756182283
0.862500000000000	4.40233394589244
0.875000000000000	4.48460105699640
0.887500000000000	4.51052014966650
0.900000000000000	4.54358710057109
0.912500000000000	4.58560438171033
0.925000000000000	4.58661637130934
0.937500000000000	4.58827972101612
0.950000000000000	4.66883166664828
0.962500000000000	4.73185071770007
0.975000000000000	4.79154762109999
0.987500000000000	4.85802016234586
1	4.90780115220246

==> Data/cdfs/50m_esprit.tex <==
0	3.60447670006024
0.0125000000000000	3.60447670006024
0.0249999999999999	3.94984029578929
0.0374999999999999	4.10196833899725
0.0499999999999998	4.15017220208623
0.0624999999999999	4.19321983168401
0.0749999999999998	4.23627920107826
0.0874999999999998	4.25366769133221
0.0999999999999999	4.25446172630460
0.112500000000000	4.26262355297481
0.125000000000000	4.27891505442321
0.137500000000000	4.28560490968531
0.150000000000000	4.30061865973781
0.162500000000000	4.31701276174946
0.175000000000000	4.31886492702317
0.187500000000000	4.31897057845093
0.200000000000000	4.33544709618323
0.212500000000000	4.35350210602568
0.225000000000000	4.38522249919880
0.237500000000000	4.42512150509991
0.250000000000000	4.42731853065433
0.262500000000000	4.43301186047226
0.275000000000000	4.44246039059048
0.287500000000000	4.45392158054424
0.300000000000000	4.46112195253256
0.312500000000000	4.46197259067609
0.325000000000000	4.46225534552972
0.337500000000000	4.46682278291902
0.350000000000000	4.47004649444259
0.362500000000000	4.47586641440659
0.375000000000000	4.47763108517343
0.387500000000000	4.49314826440783
0.400000000000000	4.49644922895799
0.412500000000000	4.50214683104671
0.425000000000000	4.50719438442595
0.437500000000000	4.52287655557599
0.450000000000000	4.52782150647210
0.462500000000000	4.52929844638935
0.475000000000000	4.54227025186088
0.487500000000000	4.55044206569370
0.500000000000000	4.55114548084822
0.512500000000000	4.55371664636382
0.525000000000000	4.55429662212821
0.537500000000000	4.56047637838642
0.550000000000000	4.56070307989927
0.562500000000000	4.56289452449594
0.575000000000000	4.56368931251569
0.587500000000000	4.56809323062606
0.600000000000000	4.58249767598196
0.612500000000000	4.58331800488834
0.625000000000000	4.60031450353759
0.637500000000000	4.62484431434065
0.650000000000000	4.62673831710787
0.662500000000000	4.64020020977316
0.675000000000000	4.64070601694107
0.687500000000000	4.64337302786987
0.700000000000000	4.64522699780216
0.712500000000000	4.64523370936121
0.725000000000000	4.64811885104448
0.737500000000000	4.65035889891985
0.750000000000000	4.66603069837247
0.762500000000000	4.67688144540771
0.775000000000000	4.67787137452346
0.787500000000000	4.67819123872055
0.800000000000000	4.67919606796394
0.812500000000000	4.69320799793640
0.825000000000000	4.70597676539207
0.837500000000000	4.71702747723871
0.850000000000000	4.72164427310058
0.862500000000000	4.73433393611114
0.875000000000000	4.73540000000000
0.887500000000000	4.73728882155049
0.900000000000000	4.75914896388538
0.912500000000000	4.78606177319127
0.925000000000000	4.78963401062138
0.937500000000000	4.79946225881390
0.950000000000000	4.80059287847281
0.962500000000000	4.82449716715970
0.975000000000000	4.82861982611044
0.987500000000000	4.98330293510931
1	5.10377498812127

==> Data/cdfs/50m_music.tex <==
0	3.62500000000000
0.0125000000000000	3.62500000000000
0.0249999999999999	3.97363636363636
0.0374999999999999	4.10636363636363
0.0499999999999998	4.15727272727273
0.0624999999999999	4.20909090909091
0.0749999999999998	4.21818181818182
0.0874999999999998	4.24545454545455
0.0999999999999999	4.25454545454546
0.112500000000000	4.25888888888889
0.125000000000000	4.26818181818182
0.137500000000000	4.26900000000000
0.150000000000000	4.27181818181818
0.162500000000000	4.28090909090909
0.175000000000000	4.32090909090909
0.187500000000000	4.34545454545454
0.200000000000000	4.34727272727273
0.212500000000000	4.37000000000000
0.225000000000000	4.38900000000000
0.237500000000000	4.39090909090909
0.250000000000000	4.43777777777778
0.262500000000000	4.43818181818182
0.275000000000000	4.44090909090909
0.287500000000000	4.44272727272727
0.300000000000000	4.44636363636364
0.312500000000000	4.46200000000000
0.325000000000000	4.46500000000000
0.337500000000000	4.46600000000000
0.350000000000000	4.47090909090909
0.362500000000000	4.47500000000000
0.375000000000000	4.47727272727273
0.400000000000000	4.48000000000000
0.412500000000000	4.48300000000000
0.425000000000000	4.49363636363636
0.437500000000000	4.50000000000000
0.450000000000000	4.50400000000000
0.462500000000000	4.50700000000000
0.475000000000000	4.52818181818182
0.487500000000000	4.55272727272727
0.500000000000000	4.55333333333333
0.512500000000000	4.55454545454546
0.525000000000000	4.55727272727273
0.537500000000000	4.55818181818182
0.550000000000000	4.56400000000000
0.562500000000000	4.56545454545455
0.575000000000000	4.56636363636364
0.587500000000000	4.57181818181818
0.600000000000000	4.58090909090909
0.612500000000000	4.58545454545455
0.625000000000000	4.61090909090909
0.637500000000000	4.61181818181818
0.650000000000000	4.61300000000000
0.662500000000000	4.61909090909091
0.675000000000000	4.62333333333333
0.687500000000000	4.62800000000000
0.712500000000000	4.64181818181818
0.725000000000000	4.64272727272727
0.737500000000000	4.64727272727273
0.750000000000000	4.65272727272727
0.762500000000000	4.66363636363637
0.775000000000000	4.67636363636364
0.787500000000000	4.67727272727273
0.800000000000000	4.67818181818182
0.812500000000000	4.69272727272727
0.825000000000000	4.69300000000000
0.837500000000000	4.69363636363636
0.850000000000000	4.71272727272728
0.862500000000000	4.71363636363636
0.875000000000000	4.73450000000000
0.887500000000000	4.73571428571429
0.900000000000000	4.76777777777778
0.912500000000000	4.76818181818182
0.925000000000000	4.78555555555556
0.937500000000000	4.79363636363636
0.950000000000000	4.82363636363636
0.962500000000000	4.82636363636364
0.975000000000000	4.86250000000000
0.987500000000000	4.98272727272727
1	5.08600000000000

==> Data/cdfs/80m_2desprit.tex <==
0	1.06248236008930
0.0125000000000000	1.06248236008930
0.0249999999999999	2.19517613117273
0.0374999999999999	2.42979058102882
0.0499999999999998	2.43300690312876
0.0624999999999999	2.48709752507432
0.0749999999999998	2.49360669021347
0.0874999999999998	2.72047575667169
0.0999999999999999	2.81750197101531
0.112500000000000	2.96580856098798
0.125000000000000	3.01145039895184
0.137500000000000	3.08365077475860
0.150000000000000	3.08654475709221
0.162500000000000	3.09210609965161
0.175000000000000	3.10810745946427
0.187500000000000	3.11233252731867
0.200000000000000	3.11779092083598
0.212500000000000	3.21237936175378
0.225000000000000	3.22403358324142
0.237500000000000	3.27887917777404
0.250000000000000	3.31896885740369
0.262500000000000	3.33562762741382
0.275000000000000	3.37008204736310
0.287500000000000	3.38552156984948
0.300000000000000	3.39495145255349
0.312500000000000	3.41003693564413
0.325000000000000	3.41354262980493
0.337500000000000	3.41923848480247
0.350000000000000	3.43624964223651
0.362500000000000	3.44321434307077
0.375000000000000	3.46659414684719
0.387500000000000	3.47408774835909
0.400000000000000	3.47647576832630
0.412500000000000	3.47753091411020
0.425000000000000	3.48445034186197
0.437500000000000	3.49730579112514
0.450000000000000	3.50021588105247
0.462500000000000	3.52905718712073
0.475000000000000	3.53238209726751
0.487500000000000	3.53545432554335
0.500000000000000	3.59622543150721
0.512500000000000	3.59899840836075
0.525000000000000	3.63448734073336
0.537500000000000	3.69592007551940
0.550000000000000	3.69788614365830
0.562500000000000	3.73769972593250
0.575000000000000	3.74269284401211
0.587500000000000	3.74489859272001
0.600000000000000	3.77626430384768
0.612500000000000	3.78458967948323
0.625000000000000	3.78819776120212
0.637500000000000	3.81567685585840
0.650000000000000	3.81642750711930
0.662500000000000	3.86924909982182
0.675000000000000	3.88498003165722
0.687500000000000	3.88924065661742
0.700000000000000	3.89397590153383
0.712500000000000	3.89495146956770
0.725000000000000	3.89581862837338
0.737500000000000	3.89588957350659
0.750000000000000	3.92552325556398
0.762500000000000	3.95823640321030
0.775000000000000	3.96626835209007
0.787500000000000	4.00302627467579
0.800000000000000	4.07453976981720
0.812500000000000	4.08728224617423
0.825000000000000	4.21284217781845
0.837500000000000	4.22276849950702
0.850000000000000	4.24097022423796
0.862500000000000	4.33191548834789
0.875000000000000	4.34478118613503
0.887500000000000	4.46976529578237
0.900000000000000	4.51039917947895
0.912500000000000	4.57317222467160
0.925000000000000	4.67228620177525
0.937500000000000	4.69588692534678
0.950000000000000	4.71711178125646
0.962500000000000	4.81034372419285
0.975000000000000	4.96057641386893
0.987500000000000	5.31363321812558
1	9.65351300676893

==> Data/cdfs/80m_esprit.tex <==
0	2.34030506421543
0.0125000000000000	2.34030506421543
0.0249999999999999	2.81095458888319
0.0374999999999999	3.05715430715145
0.0499999999999998	3.19646253491964
0.0624999999999999	3.38373843632201
0.0749999999999998	3.43378458262739
0.0874999999999998	3.62804953720958
0.0999999999999999	3.77667318166000
0.112500000000000	3.82832716603568
0.125000000000000	3.89185489768505
0.137500000000000	3.93425465769167
0.150000000000000	3.93516845385708
0.162500000000000	3.95799533176541
0.175000000000000	4.00265667937683
0.187500000000000	4.01544596322502
0.200000000000000	4.11335966993604
0.212500000000000	4.17178279579386
0.225000000000000	4.18780961198771
0.237500000000000	4.34938013052332
0.250000000000000	4.46570039694429
0.262500000000000	4.49460687248277
0.275000000000000	4.53498562439822
0.287500000000000	4.58343596138342
0.300000000000000	4.64314547989457
0.312500000000000	4.68288505368634
0.325000000000000	4.70228365330555
0.337500000000000	4.70422212613385
0.350000000000000	4.70659722088364
0.362500000000000	4.71510309421865
0.375000000000000	4.72001045714580
0.387500000000000	4.74922685275776
0.400000000000000	4.78223263620334
0.412500000000000	4.79177575700110
0.425000000000000	4.79891905971508
0.437500000000000	4.81498896547124
0.450000000000000	4.85393681825607
0.462500000000000	4.87610194699776
0.475000000000000	4.89353818577990
0.487500000000000	4.92895671378928
0.500000000000000	4.93534744645220
0.512500000000000	4.94286096317970
0.525000000000000	5.00762534776874
0.537500000000000	5.02902037290017
0.550000000000000	5.04716689826841
0.562500000000000	5.05858192948130
0.575000000000000	5.06566409819879
0.587500000000000	5.07601514161971
0.600000000000000	5.13683508158538
0.612500000000000	5.14991928332128
0.625000000000000	5.23410731844765
0.637500000000000	5.24053898357754
0.650000000000000	5.24644277122066
0.662500000000000	5.28856654534035
0.675000000000000	5.29191413449744
0.687500000000000	5.32482984781226
0.700000000000000	5.32784991441168
0.712500000000000	5.41345024281813
0.725000000000000	5.43577586748701
0.737500000000000	5.52098813394657
0.750000000000000	5.60718308843777
0.762500000000000	5.60780610220566
0.775000000000000	6.00238238295288
0.787500000000000	6.08385937561484
0.800000000000000	6.09246763477721
0.812500000000000	6.33537508392643
0.825000000000000	6.38370611229543
0.837500000000000	6.40598077590641
0.850000000000000	6.53900357298640
0.862500000000000	6.60874198129323
0.875000000000000	6.86888143118232
0.887500000000000	6.87982228958713
0.900000000000000	7.08043073134516
0.912500000000000	8.06913759625278
0.925000000000000	8.38102673182751
0.937500000000000	27.9230578697434
0.950000000000000	28.6595808358923
0.962500000000000	38.9887042330679
0.975000000000000	44.0398699532436
0.987500000000000	45.3107804603449
1	49.0087990780002

==> Data/cdfs/80m_music.tex <==
0	2.34700000000000
0.0125000000000000	2.34700000000000
0.0249999999999999	2.82272727272727
0.0374999999999999	3.00181818181818
0.0499999999999998	3.06000000000000
0.0624999999999999	3.39666666666667
0.0749999999999998	3.44700000000000
0.0874999999999998	3.63750000000000
0.0999999999999999	3.78888888888889
0.112500000000000	3.85818181818182
0.125000000000000	3.90454545454545
0.137500000000000	3.94363636363636
0.150000000000000	3.97300000000000
0.162500000000000	4.01750000000000
0.175000000000000	4.04181818181818
0.187500000000000	4.06200000000000
0.200000000000000	4.14200000000000
0.212500000000000	4.19454545454545
0.225000000000000	4.21100000000000
0.237500000000000	4.35454545454546
0.250000000000000	4.47900000000000
0.262500000000000	4.52363636363636
0.275000000000000	4.54272727272727
0.287500000000000	4.59909090909091
0.300000000000000	4.70727272727272
0.312500000000000	4.71300000000000
0.325000000000000	4.71909090909091
0.337500000000000	4.72400000000000
0.350000000000000	4.73363636363636
0.362500000000000	4.73727272727273
0.375000000000000	4.76818181818182
0.387500000000000	4.80000000000000
0.400000000000000	4.81545454545454
0.412500000000000	4.82625000000000
0.425000000000000	4.84909090909091
0.437500000000000	4.92181818181818
0.450000000000000	4.94000000000000
0.462500000000000	4.94181818181818
0.475000000000000	4.95090909090909
0.487500000000000	4.99300000000000
0.500000000000000	4.99900000000000
0.512500000000000	5.03090909090909
0.525000000000000	5.05363636363637
0.537500000000000	5.07125000000000
0.550000000000000	5.07888888888889
0.562500000000000	5.11375000000000
0.575000000000000	5.13000000000000
0.587500000000000	5.14818181818182
0.600000000000000	5.16000000000000
0.612500000000000	5.16800000000000
0.625000000000000	5.24375000000000
0.637500000000000	5.24909090909091
0.650000000000000	5.28600000000000
0.662500000000000	5.30090909090909
0.675000000000000	5.32250000000000
0.687500000000000	5.33000000000000
0.700000000000000	5.41636363636364
0.712500000000000	5.48333333333334
0.725000000000000	5.54363636363636
0.737500000000000	5.55100000000000
0.750000000000000	5.63727272727273
0.762500000000000	5.63900000000000
0.775000000000000	6.08454545454545
0.787500000000000	6.11909090909091
0.800000000000000	6.35111111111111
0.812500000000000	6.38333333333333
0.825000000000000	6.46454545454546
0.837500000000000	6.47363636363636
0.850000000000000	6.62000000000000
0.862500000000000	6.87800000000000
0.875000000000000	7.08400000000000
0.887500000000000	7.41000000000000
0.900000000000000	7.58750000000000
0.912500000000000	7.64181818181818
0.925000000000000	8.38454545454545
0.937500000000000	8.44090909090909
0.950000000000000	22.4854545454545
0.962500000000000	23.5336363636364
0.975000000000000	26.9254545454545
0.987500000000000	34.5870000000000
1	44.2988888888889

==> Data/crb0.tex <==
-5 0.169977697883756
-4 0.162529905123315
-3 0.155050902908407
-2 0.149435346783153
-1 0.140845982241632
0 0.133008371349980
1 0.125798804359954
2 0.117246781649741
3 0.107025061021797
4 0.0985510055614626
5 0.0913328659316833
6 0.0827513719853009
7 0.0737909610732668
8 0.0678685398433093
9 0.0598828236108399
10 0.0540980598219508

==> Data/crb0mp3.tex <==
-5	0.597596827918866
-4	0.562749702864373
-3	0.523675016071905
-2	0.482582127725289
-1	0.448211562236877
0	0.407993530157015
1	0.379859834730052
2	0.347812926981762
3	0.310729093752093
4	0.280062248375054
5	0.255262870213955
6	0.231024032942594
7	0.205562656990341
8	0.179322626285684
9	0.161403010999578
10	0.145586141879576

==> Data/crb45.tex <==
-5 0.242636210910518
-4 0.231891230708486
-3 0.220184189966772
-2 0.210483754875967
-1 0.20009400858864
0 0.189597655749466
1 0.176822937879687 
2 0.166371845320905 
3 0.152333567734854
4 0.140105655493142
5 0.129080500579412
6 0.114725761189433
7 0.105879195990704
8 0.0952825313922271
9 0.0852187400401731
10 0.0771974586184616

==> Data/football_field.tex <==
1	-1.25800000000000	-1.25846222809465	-0.213186909726134	-4.73450000000000	-4.73540000000000	-4.58661637130934	4.35454545454546	4.34938013052332	4.57317222467160
2	-1.04545454545454	-1.04620382455751	-0.0173514494329170	-4.66363636363637	-4.66603069837247	-3.78981591102129	6.46454545454546	6.00238238295288	2.49360669021347
3	-1.45818181818182	-1.45796308663973	-0.408434049506953	-3.62500000000000	-3.60447670006024	-3.56152655061659	4.59909090909091	4.58343596138342	3.39495145255349
4	-1.35909090909091	-1.35888598793572	-0.536184514870704	-4.49363636363636	-4.49314826440783	-3.87310315850133	4.19454545454545	4.17178279579386	4.33191548834789
5	-1.42272727272727	-1.42191571519607	-0.429816344063765	-4.61300000000000	-4.64020020977316	-4.37256756182283	6.62000000000000	6.60874198129323	3.88498003165722
6	-1.28200000000000	-1.28025314183806	-0.589079134388514	-4.43818181818182	-4.42731853065433	-3.66749987501031	4.54272727272727	4.53498562439822	3.10810745946427
7	-1.02625000000000	-0.998218134418824	-0.125251400369511	-4.57181818181818	-4.56809323062606	-4.54358710057109	5.13000000000000	5.07601514161971	3.49730579112514
8	-1.33222222222222	-1.33112345840064	-0.636859541604748	-4.25454545454546	-4.25446172630460	-4.07892711664446	7.41000000000000	6.40598077590641	2.72047575667169
9	-1.38600000000000	-1.38735160544191	-0.413429937625065	-4.44090909090909	-4.44246039059048	-3.78545529999951	5.07888888888889	5.04716689826841	3.50021588105247
10	-1.37000000000000	-1.36988706318064	-0.720824848543645	-4.34727272727273	-4.33544709618323	-3.72109075567052	8.44090909090909	8.06913759625278	3.21237936175378
11	-1.01555555555556	-1.01669034490398	-0.116170241549362	-4.47727272727273	-4.46197259067609	-4.08922043246139	6.47363636363636	6.38370611229543	3.09210609965161
12	-1.39363636363637	-1.39424721998348	-0.562977442582494	-4.61909090909091	-4.73728882155049	-3.90088289759810	4.04181818181818	4.01544596322502	3.44321434307077
13	-1.66727272727273	-1.66936669798632	-0.943092292425773	-4.50000000000000	-4.50214683104671	-3.90767596437161	3.44700000000000	3.43378458262739	3.96626835209007
14	-1.16200000000000	-1.16290203956682	-0.333187377539175	-4.55333333333333	-4.54227025186088	-3.96379425179844	7.08400000000000	7.08043073134516	3.41003693564413
15	-1.44727272727273	-1.40746916897199	-0.589279773593410	-4.21818181818182	-4.30061865973781	-4.11883056557276	4.81545454545454	4.79177575700110	3.95823640321030
16	-1.90800000000000	-1.90782670116149	-0.550314134498542	-4.82636363636364	-4.82861982611044	-3.67936490493416	3.85818181818182	3.82832716603568	3.92552325556398
17	-1.32727272727273	-1.32701833701642	-0.395950874634260	-4.73571428571429	-4.73433393611114	-3.88393083588726	4.80000000000000	4.64314547989457	3.41354262980493
18	-1.23818181818182	-1.23740629560999	-0.395055953212876	-4.65272727272727	-4.65035889891985	-3.85774561055024	4.76818181818182	4.74922685275776	3.52905718712073
19	-1.27800000000000	-1.25547177490045	-0.338662857642352	-4.38900000000000	-4.42512150509991	-4.73185071770007	5.11375000000000	5.06566409819879	3.69788614365830
20	-1.45272727272727	-1.45381638301717	-0.365092183784310	-4.78555555555556	-4.80059287847281	-4.85802016234586	4.52363636363636	4.49460687248277	3.63448734073336
21	-1.62272727272727	-1.62150222917589	-0.794465643360891	-4.64727272727273	-4.64811885104448	-3.80654867505986	5.24375000000000	4.81498896547124	3.81567685585840
22	-1.18090909090909	-1.17933790321378	-0.314579788937948	-4.44272727272727	-4.43301186047226	-3.91696397486300	4.73363636363636	4.72001045714580	4.07453976981720
23	-1.23000000000000	-1.23149462943838	-0.435332609737782	-4.98272727272727	-4.98330293510931	-4.21579151642234	4.70727272727272	4.68288505368634	4.08728224617423
24	-1.34727272727273	-1.34713727763771	-0.482803424406822	-4.64272727272727	-4.64522699780216	-3.94849715261309	5.24909090909091	5.23410731844765	3.78819776120212
25	-1.42636363636364	-1.42814119633481	-0.532310958505830	-4.69272727272727	-4.69320799793640	-4.04131552460727	4.71300000000000	4.70228365330555	3.77626430384768
26	-1.22181818181818	-1.22246378829102	-0.333914791104194	-3.97363636363636	-3.94984029578929	-3.68285378244185	6.11909090909091	6.09246763477721	3.11779092083598
27	-1.41400000000000	-1.41343028851332	-0.606843330618138	-4.43777777777778	-4.52287655557599	-3.55494627094893	5.54363636363636	5.52098813394657	3.37008204736310
28	-1.19636363636364	-1.19602482791397	-0.347584790786024	-4.26900000000000	-4.31886492702317	-4.12816329716527	5.63727272727273	5.60780610220566	3.89495146956770
29	-1.28545454545455	-1.28563299382057	-0.475030315455840	-4.50700000000000	-4.50719438442595	-3.73444850425620	6.35111111111111	6.33537508392643	3.33562762741382
30	-1.17285714285714	-1.17269521818719	-0.414619572728202	-4.76777777777778	-4.78963401062138	-4.35563951610627	4.47900000000000	4.46570039694429	3.43624964223651
31	-1.15333333333333	-1.15315734363218	-0.513798865682586	-4.71363636363636	-4.71702747723871	-4.09292747148530	4.71909090909091	4.70659722088364	4.51039917947895
32	-1.03818181818182	-1.03943567622220	-0.111957618749536	-4.55818181818182	-4.56047637838642	-4.04766709880514	5.33000000000000	5.32482984781226	4.00302627467579
33	-1.49800000000000	-1.49751163901413	-0.0903122653115222	-4.64181818181818	-4.64337302786987	-4.10552175921205	4.99300000000000	4.89353818577990	4.34478118613503
34	-1.01000000000000	-1.01006904839976	-0.332154781734780	-4.71272727272728	-4.70597676539207	-3.87139036624435	4.72400000000000	4.70422212613385	3.86924909982182
35	-1.13727272727272	-1.13815720701791	-0.204723800947581	-4.28090909090909	-4.27891505442321	-3.99919433756670	3.94363636363636	3.93516845385708	4.21284217781845
36	-1.14181818181818	-1.14119710837800	-0.562172232372947	-4.15727272727273	-4.15017220208623	-3.89606015520538	3.97300000000000	3.95799533176541	3.74489859272001
37	-1.15800000000000	-1.15734668343286	-0.528920530967022	-4.10636363636363	-4.10196833899725	-3.88987815156188	5.07125000000000	5.05858192948130	4.71711178125646
38	-1.25636363636364	-1.25716601197090	-0.272238066949407	-4.86250000000000	-4.78606177319127	-4.12358117181888	7.64181818181818	6.87982228958713	3.73769972593250
39	-1.23909090909091	-1.23800303983381	-0.369122257025348	-4.47500000000000	-4.47586641440659	-3.87292726280269	4.14200000000000	4.11335966993604	3.69592007551940
40	-1.35272727272727	-1.35330715661786	-0.320850784731072	-4.46200000000000	-4.46225534552972	-3.96917805563014	5.14818181818182	5.13683508158538	2.43300690312876
41	-1.25545454545454	-1.25522315862126	-0.00882814690755306	-4.64181818181818	-4.64523370936121	-3.94573223522007	2.82272727272727	2.81095458888319	3.89581862837338
42	-1.33454545454546	-1.33692571085930	-0.316472953455095	-4.61181818181818	-4.62673831710787	-4.58560438171033	7.58750000000000	27.9230578697434	2.42979058102882
43	-1.49363636363636	-1.49432321125450	-0.349752952362325	-4.50400000000000	-4.55044206569370	-4.05453949550687	5.41636363636364	5.41345024281813	3.81642750711930
44	-1.33909090909091	-1.34092688859100	-0.296618763824755	-4.67818181818182	-4.67688144540771	-4.01913054395638	44.2988888888889	49.0087990780002	1.06248236008930
45	-1.60363636363636	-1.60431321938328	-0.800545283155272	-4.46500000000000	-4.49644922895799	-3.89440386048161	5.48333333333334	5.43577586748701	3.01145039895184
46	-1.17090909090909	-1.17021172635563	-0.238124471067589	-4.46600000000000	-4.46682278291902	-3.70834801274957	4.94181818181818	4.94286096317970	4.67228620177525
47	-1.16545454545454	-1.16488195375566	-0.426978422719192	-4.39090909090909	-4.38522249919880	-3.74876002725482	3.00181818181818	3.19646253491964	3.47647576832630
48	-1.07363636363636	-1.07185689693694	-0.0701743441194497	-4.20909090909091	-4.19321983168401	-3.79685448901720	6.08454545454545	6.08385937561484	3.53545432554335
49	-1.31545454545454	-1.31475449552195	-0.879574905941431	-4.62800000000000	-4.64070601694107	-3.86841221503547	3.06000000000000	3.05715430715145	5.31363321812558
50	-1.39363636363636	-1.39500533193983	-0.751416759620127	-4.56400000000000	-4.56070307989927	-3.87307613485699	5.03090909090909	5.00762534776874	3.47408774835909
51	-1.70818181818182	-1.70758968342809	-0.886218669664113	-4.62333333333333	-4.62484431434065	-3.87351573239003	3.90454545454545	3.89185489768505	3.11233252731867
52	-1.42090909090909	-1.42089861070247	-0.901188064676355	-4.44636363636364	-4.45392158054424	-3.53601865274128	2.34700000000000	2.34030506421543	3.89588957350659
53	-1.31400000000000	-1.31385022094629	-0.532301016207248	-4.76818181818182	-4.75914896388538	-4.66883166664828	4.06200000000000	3.93425465769167	4.22276849950702
54	-1.33700000000000	-1.34315070050823	-0.478757247661224	-4.34545454545454	-4.31701276174946	-3.77618374112068	3.63750000000000	3.62804953720958	2.81750197101531
55	-1.47818181818182	-1.47858901976160	-1.05482099890778	-4.69300000000000	-4.67919606796394	-3.74133953943932	4.92181818181818	4.87610194699776	4.24097022423796
56	-1.12818181818182	-1.12808469451007	-0.551937021894638	-4.37000000000000	-4.35350210602568	-3.78995937090111	5.32250000000000	5.29191413449744	3.41923848480247
57	-1.20000000000000	-1.20055752081248	-0.349066127611547	-4.67636363636364	-4.67819123872055	-4.48460105699640	4.73727272727273	4.71510309421865	3.59899840836075
58	-1.38818181818182	-1.38834946988009	-1.12166560442352	-4.56636363636364	-4.56289452449594	-4.09540655966228	4.94000000000000	4.93534744645220	4.46976529578237
59	-1.39000000000000	-1.39105404742129	-0.490257954132213	-4.69363636363636	-4.72164427310058	-4.58827972101612	22.4854545454545	45.3107804603449	3.22403358324142
60	-1.20750000000000	-1.22243624307179	-0.522053580189122	-4.24545454545455	-4.23627920107826	-4.00484684370648	4.01750000000000	4.00265667937683	2.48709752507432
61	-1.13363636363636	-1.13330827457444	-0.483087863089054	-4.82363636363636	-4.82449716715970	-4.22632925936511	3.39666666666667	3.38373843632201	2.96580856098798
62	-1.16555555555556	-1.16409417087665	-0.413738740611538	-4.58545454545455	-4.58249767598196	-4.01910351454330	6.87800000000000	6.86888143118232	3.78458967948323
63	-1.12090909090909	-1.12061249847936	-0.0923542663587230	-4.55454545454546	-4.55371664636382	-3.85238249285174	26.9254545454545	44.0398699532436	4.96057641386893
64	-1.20090909090909	-1.20172808237705	-0.405144499578484	-4.56545454545455	-4.56368931251569	-4.40233394589244	4.99900000000000	4.85393681825607	3.59622543150721
65	-1.11600000000000	-1.11561427290737	-0.327510718071559	-4.55727272727273	-4.55429662212821	-3.76781913221341	3.78888888888889	3.77667318166000	3.27887917777404
66	-1.13700000000000	-1.13906701365557	-0.398253674695040	-4.48000000000000	-4.47763108517343	-3.76258593229942	4.84909090909091	4.78223263620334	3.38552156984948
67	-1.10090909090909	-1.10095632730110	-0.319113432436410	-4.25888888888889	-4.25366769133221	-3.98697002993921	4.82625000000000	4.79891905971508	3.88924065661742
68	-1.23400000000000	-1.22709657232275	-0.475832828740898	-4.55272727272727	-4.55114548084822	-3.86412526003144	5.63900000000000	5.60718308843777	3.46659414684719
69	-1.25909090909091	-1.25886711707377	-0.498237229525332	-4.27181818181818	-4.28560490968531	-3.91576456656673	4.21100000000000	4.18780961198771	3.31896885740369
70	-1.02400000000000	-1.02278153148013	-0.173141126779755	-4.67727272727273	-4.67787137452346	-4.51052014966650	5.28600000000000	5.24644277122066	4.69588692534678
71	-1.16888888888889	-1.14476836475236	-0.422806254229928	-4.26818181818182	-4.26262355297481	-3.60325940069063	8.38454545454545	8.38102673182751	4.81034372419285
72	-1.23363636363636	-1.23392794938995	-0.275011278807777	-4.47090909090909	-4.47004649444259	-3.66494482562497	23.5336363636364	28.6595808358923	2.19517613117273
73	-1.28363636363636	-1.28444344283582	-0.335156202918840	-4.58090909090909	-4.58331800488834	-4.03386096295606	4.95090909090909	4.92895671378928	3.89397590153383
74	-1.16500000000000	-1.14834887914542	-0.257797795541727	-4.79363636363636	-4.79946225881390	-3.48441855056768	5.16000000000000	5.32784991441168	3.47753091411020
75	-1.20909090909091	-1.21022723362472	-0.279033064880827	-5.08600000000000	-5.10377498812127	-4.90780115220246	5.30090909090909	5.28856654534035	3.53238209726751
76	-1.21428571428572	-1.19388784257747	-0.0946927285190187	-4.48000000000000	-4.46112195253256	-4.79154762109999	5.55100000000000	5.24053898357754	3.74269284401211
77	-1.09727272727273	-1.11524988272177	-0.203398721074568	-4.52818181818182	-4.52782150647210	-4.08152050400862	5.16800000000000	5.14991928332128	3.08365077475860
78	-1.07500000000000	-1.10579204205884	-0.380420941314642	-4.32090909090909	-4.31897057845093	-3.99647128397882	6.38333333333333	6.53900357298640	3.48445034186197
79	-1.16500000000000	-1.16483584262037	-0.248203066607281	-4.61090909090909	-4.60031450353759	-4.00386886082651	5.05363636363637	5.02902037290017	3.08654475709221
80	-1.24727272727273	-1.24852538894820	-0.426501816577742	-4.48300000000000	-4.52929844638935	-3.94722347761811	34.5870000000000	38.9887042330679	9.65351300676893

==> Data/mpc_15.tex <==
-5	0.351375481043989	0.722322077122498	0.745687085177153
-4	0.290266709104988	0.648347305105294	0.661740834466182
-3	0.256260884932386	0.579414122753819	0.609566448387703
-2	0.232121040047780	0.515693237156899	0.507671064765364
-1	0.193744995840567	0.421130117128131	0.489953794760281
0	0.169253471299415	0.388617471097547	0.415586106601266
1	0.145305504404064	0.356613209397351	0.374849356408677
2	0.133567691986504	0.325040893393493	0.331392015594823
3	0.120883864323271	0.301459224452118	0.333225473215958
4	0.101956483200774	0.285062631011233	0.265496751392554
5	0.0918946298668426	0.235520006599154	0.207054884028365
6	0.0815263397368228	0.220216942474971	0.221043307973799
7	0.0753048676297042	0.148023123857751	0.190535534743521
8	0.0665491500465967	0.175147149917307	0.197952486723455
9	0.0569778503687420	0.158153350177876	0.139993289124871
10	0.0521129461145243	0.111703230077761	0.133554606809349

==> results.tex <==
\label{results}
\begin{comment}
\subsection{AoA Computation}
Different scenarios are evaluated consisting of a variety of LOS AoAs, Multipath Components (MPCs) and interference from other users. For each scenario, two cases have been selected: (i) one case close to the best possible one, i.e., an AoA of 0\degree{} with a large discrepancy, indicatively more than~20\degree {}, between the LOS path and the MPCs/interference when present; and (ii) one case where source separation could have been problematic. The scenarios evaluated here, are summarized in Table~\ref{scenarios}. 500 realizations have been performed for each scenario in MATLAB, measuring the ability to discriminate user angle from the multipath effect and interference, plus the Root Mean Square Error (RMSE) of angle estimation. Since in the case of a multipath component or interference more than one Angles are estimated, there is a need to choose the angle of interest. For the MUSIC and 1D ESPRIT algorithms, the power of a beamformer at the estimated angles is measured, and the angle corresponding to the most powerful outcome of the beamformer is selected. For the 2D ESPRIT algorithm, a cross-correlation of the replica waveform for each computed pair of angle/delay is calculated, selecting the pair with the highest correlation coefficient. 
\begin{table}[t]%[!h]
\centering
\caption{Simulated Angles for LOS Path, MPCs and Interfering Users}
\label{Simulation Parameters}
\footnotesize
\begin{tabular}{lcccl}\toprule
Scenario & LOS Path & Multipath Components & Interference \\
\midrule
Scenario I & 0\degree & - & -\\ 
Scenario II & 45\degree & - & -\\
Scenario III & 0\degree & 30\degree \space and $-$30\degree & -\\ 
Scenario IV & 45\degree & 30\degree \space and 60\degree & -\\
Scenario V & 0\degree & 30\degree \space and $-$30\degree & 60\degree \space and $-$60\degree \\ 
Scenario VI & 45\degree & 5\degree \space and $-$15\degree & 25\degree \space and 65\degree \\
\bottomrule
\end{tabular}
\label{scenarios}
\end{table}
\begin{comment}
\begin{figure}[h!]%[!h]
%\begin{tabular}{cc}
        %\includestandalone[width=.48\textwidth]{ScenarioI}
        %\includestandalone[width=\columnwidth]{figs/ScenarioI}
        \input{figs/2desprit2}
 %&
    %\includestandalone[width=.22\textwidth]{ScenarioII} \\
%\end{tabular}
\caption{Evaluation of the performance of 2D ESPRIT for different stacking parameters $m_1$}
\label{parameter m1}
\end{figure}
\begin{figure}[t]%[!h]
%\begin{tabular}{cc}
        %\includestandalone[width=.48\textwidth]{ScenarioI}
        %\includestandalone[width=\columnwidth]{figs/ScenarioI}
        \input{figs/2despritextimef}
 %&
    %\includestandalone[width=.22\textwidth]{ScenarioII} \\
%\end{tabular}
\caption{Execution time of 2D ESPRIT versus stacking parameter $m_1$}
\label{extime}
\end{figure}

In \cite{2DESPRIT}, different stacking parameters $m_1$ and $m_2$ have been evaluated. A similar evaluation is  reported here %has been carried out
for our system for the stacking parameter $m_1$. Fig.~\ref{parameter m1} presents the RMSE error %in degrees 
%for the desired angle computation 
in angle estimation,
for Scenario~VI. As the CSI matrix %has dimensions 
is of size $N_{\text{subcarriers}} \times N_{\text{antennas}}$, vertically stacking $m_1$ copies of the shifted CSI matrix increases the size of the algorithm input, thus increasing the overall execution time. Fig.~\ref{extime} shows the execution time of 2D ESPRIT as a function of $m_1$. It is found that $m_1 = 5$, i.e., stacking  five shifted copies of the CSI matrix, for $m_2 = 1$ is a well-balanced case for performance versus execution time; thus it is adopted in our simulations.  
All the results refer to Configuration 1 of Table~\ref{Configuration}. Regarding the multipath components, the first angle is simulated having half of the LOS path power, while the second angle has a third of the LOS path power. For interference, two additional SRS sequences, scrambled differently than the original are transmitted. The first angle refers to a user transmitting in different subcarriers, while the second angle refers to a user transmitting in the same subcarriers. Both users transmit at a third of the LOS path power. 
\begin{figure}[t]%[!h]
%\begin{tabular}{cc}
        %\includestandalone[width=.48\textwidth]{ScenarioI}
        %\includestandalone[width=\columnwidth]{figs/ScenarioI}
        \input{figs/ScenarioI}
 %&
    %\includestandalone[width=.22\textwidth]{ScenarioII} \\
%\end{tabular}
\caption{RMSE Error in degrees for Scenario I}
\label{LOS Scenario I}
\end{figure}
\begin{figure}[t]%!h]
%\begin{tabular}{cc}
        \input{figs/ScenarioII}

        %\includestandalone[width=.48\textwidth]{ScenarioII}
 %&
    %\includestandalone[width=.22\textwidth]{ScenarioII} \\
%\end{tabular}
\caption{RMSE Error in degrees for Scenario II}
\label{LOS Scenario II}
\end{figure}
\begin{figure}[!h]%!h]
%\begin{tabular}{cc}
        \input{figs/ScenarioIII}

        %\includestandalone[width=.48\textwidth]{ScenarioIII}
 %&
 %   \includestandalone[width=.22\textwidth]{ScenarioIV} \\
%\end{tabular}
\caption{RMSE Error in degrees for Scenario~III}
\label{MPC Scenario I}
\end{figure}
\begin{figure}[!h]
        \input{figs/ScenarioIV}

%\begin{tabular}{cc}
 %       \includestandalone[width=.48\textwidth]{ScenarioIV}
 %&
 %   \includestandalone[width=.22\textwidth]{ScenarioIV} \\
%\end{tabular}
\caption{RMSE Error in degrees for Scenario IV}
\label{MPC Scenario II}
\end{figure}
\begin{figure}[!ht]
%\begin{tabular}{cc}
        \input{figs/ScenarioV}

        %\includestandalone[width=.48\textwidth]{ScenarioV}
 %&
 %   \includestandalone[width=.22\textwidth]{ScenarioVI} \\
%\end{tabular}
\caption{RMSE Error in degrees for Scenario~V}
\label{MPCI Scenarios I}
\end{figure}

\begin{figure}[!h]
%\begin{tabular}{cc}
        \input{figs/ScenarioVI}

        %\includestandalone[width=.48\textwidth]{ScenarioVI}
 %&
 %   \includestandalone[width=.22\textwidth]{ScenarioVI} \\
%\end{tabular}
\caption{RMSE Error in degrees for Scenario VI}
\label{MPCI Scenarios II}
\end{figure}
%\begin{figure}[!h]
%\begin{tabular}{cc}
%        \includestandalone[width=.22\textwidth]{ScenarioVhits}
% &
%    \includestandalone[width=.22\textwidth]{ScenarioVIhits} \\
%\end{tabular}
%\caption{Percentage of desired angle selection for Scenarios V and VI}
%\label{MPCI Scenarios hits}
%\end{figure}

\begin{figure}[!h]
%\begin{tabular}{cc}
        \input{figs/LOSScenariohits}

        %\includestandalone[width=.48\textwidth]{LOSScenariohits}
 %&
 %   \includestandalone[width=.22\textwidth]{ScenarioIhits} \\
%\end{tabular}
\caption{Percentage of desired angle selection for Scenarios~I and~II}
\label{LOS Scenarios hits}
\end{figure}

\begin{figure}[t]%[!h]
%\begin{tabular}{cc}
\input{figs/MPCScenariohits}
        %\includestandalone[width=.48\textwidth]{MPCScenariohits}
 %&
 %   \includestandalone[width=.22\textwidth]{ScenarioIVhits} \\
%\end{tabular}
\caption{Percentage of desired angle selection for Scenarios~III and~IV}
\label{MPC Scenarios hits}
\end{figure}

\begin{figure}[!h]%[!h]
\input{figs/ScenarioMPCI}

%\includestandalone[width=.48\textwidth]{ScenarioMPCI}
\caption{Percentage of desired angle selection for Scenarios~V and~VI}
\label{MPCI Scenarios hits}
\end{figure}
Figs.~\ref{LOS Scenario I}--\ref{MPCI Scenarios II} show the RMSE \emph{vs.} SNR for each of the scenarios of Table~\ref{scenarios}. Figs.~\ref{LOS Scenarios hits} and~\ref{MPC Scenarios hits} present the percentage of the desired user angle selection for each scenario. Specifically for Figs.~\ref{MPCI Scenarios I}, \ref{MPCI Scenarios II} and \ref{MPCI Scenarios hits} it is noted that although there is interference present, the results are plotted for the target SNR for a more direct comparison with the rest of the scenarios. Plotting versus the SINR would result in an horizontal translation of the curves. For Scenarios III--VI (corresponding to Fig.~\ref{parameter m1}, Figs.~\ref{MPC Scenario I}--\ref{MPCI Scenarios II}), the presented Cramer Rao Bound is computed without cosnidering the MPCs or interference. 

Simulation results show that the 2D ESPRIT is the algorithm with the best overall performance, especially in the presence of interference. As the input of the aforementioned algorithm is not raw data but the CSI matrix, the knowledge of the training sequence is exploited, filtering out a portion of the unwanted signals. It can also be noted that MUSIC and 1D ESPRIT perform in a very similar manner in both the angular estimation and the desired angle computation, something that was expected, but nevertheless confirmed. Fig.~\ref{MPC Scenario II} presents a special case, as the angles of the received signals are too close to be distinguished by the estimator.

\subsection{Execution Time}
Since the simulations are targeted to an SDR application, the complexity of the algorithms can be related to their execution time, which is comparatively  evaluated for the various cases, in MATLAB. The simulations were performed on an Intel Xeon Silver 4214@2.2 GHz processor, on a server running CentOS~8 with 128~GB RAM. %The obtained results are summarized 
Table~\ref{Execution Time} summarizes the obtained results.
As Table~\ref{Execution Time} shows, the 1D ESPRIT is the algorithm with the least amount of computational burden, as the AoA estimation is performed in closed form. The case of 2D ESPRIT is slightly different, as a 2D matrix is processed and therefore requires additional computational effort. However, the overall computational load of 2D ESPRIT can be accommodated by the target testbed. 
%The MUSIC algorithm searches for a peak in its spectrum with a step of~0.01\degree \space in line with the Cramer-Rao Bound. It can be optimized accordingly to further reduce its execution time. 
The MUSIC algorithm searches for a peak in its spectrum with a step of~0.01\degree \space so that its performance is in line with the Cramer-Rao Bound. It can be optimized accordingly to further reduce its execution time. 
\begin{table}[tb]%[!h]
\centering
\caption{Execution time %in seconds 
for 2D ESPRIT, MUSIC and 1D ESPRIT}
\label{Execution Time}
\footnotesize
\begin{tabular}{lcl}
\toprule
Algorithm & Execution Time (s) \\
\midrule
2D ESPRIT (*) & 0.008 \\
MUSIC (**) & 0.07 \\
1D ESPRIT & 0.0004 \\
\bottomrule
\multicolumn{2}{l}{
(*) for $m_1 = 5$ \hskip3em
(**) with a search step of 0.01\degree
}
\end{tabular}
\end{table}
\end{comment}

==> signal_reception.tex <==
\label{reception}
Assuming an $M$-element ULA, $M$ copies of the signal $x_{\text{chan}}(t)$ propagate through the channel and are received, one per antenna element, having the form
\begin{equation}
    x(t) = \sum_{p=1}^{P} \mathbf{A}(\theta_p)D_p(t) s(t-\tau_p) + n(t),
    \label{signal_reception}
\end{equation}
where $\mathbf{A}(\theta_p$) is the steering vector of the $p$-th path, 
%Assuming an $M$-element ULA, $M$ copies of the signal $y(t)$ propagate through the channel and are received, one for each antenna element. Signal copies have a very small relative delay~$\tau_m$ , and are expressed as
%\begin{equation}
%        \mathbf{Y_m} = \begin{bmatrix}
%        y_{\text{chan}}(t)\\
%        y_{\text{chan}}(t-\tau_m)\\
%        \vdots\\
%        y_{\text{chan}}(t-(M-1) \tau_m)
%    \end{bmatrix}
%    \label{delay}
%\end{equation}

%Since the Narrowband assumption is satisfied $(B\Delta T \ll 1)$ where $B$ is the bandwidth and $\Delta T$ is the time difference of arrival of the plane wave between two sensors of the array, it can be assumed that the array outputs only differ by a phase shift. With respect to the origin, \eqref{delay} can be rewritten as
\begin{equation}
       \mathbf{A}(\theta_p) = \begin{bmatrix}
        1\\
        \exp\left({\frac{-j2\pi f_c d \sin{\theta_p}}{c}}\right)\\
        \vdots\\
        \exp\left({\frac{-j2\pi f_c (M-1) d \sin{\theta_p}}{c}}\right)\\
    \end{bmatrix},
    \label{steering}
\end{equation}
where $f_c$ is the carrier frequency, $d$ is the antenna element spacing, $c$ is the speed of light, and $\theta_p$ is the azimuth angle of path $p$. 

\subsection{Timing Synchronization}
The receiver computes the offset of the received waveform in samples using cross-correlation, as it is stored locally and unaffected by noise. The offset, relative to the original waveform, is determined as the as the index $n^*$ corresponding to the largest peak of the cross-correlation output $c(n)$.
\begin{align}
n^* = \operatorname{argmax} c(n),
\intertext{where}
c(n) = \sum_{i=1}^{L_{\text{seq}} -1} s^*(i) x(n+i),
\end{align}
%and %$i$ denotes the time domain samples,
$L_{\text{seq}}$ denotes the length of the transmitted waveform in samples and $s^*$ denotes the conjugate of $s$.

\subsection{Estimating the Correct Number of Paths}
The super-resolution algorithms, i.e., MUSIC, ESPRIT, require a knowledge of the number of sources (or, in our case, the number of received, reflected paths). Several prior studies addressed this topic \cite{Ivan}, \cite{Cheng}. An underperformance of the algorithms occurs when the number of sources is not correctly estimated.
%For this scope, 
In the following, three techniques for the estimation of the number of sources are comparatively evaluated, namely
the Akaike Information Criterion (AIC) \cite{Akaike}, Minimum Description Length (MDL)~\cite{MDL} and Efficient Channel Order Determination Method (ECOD)~\cite{ECOD}, 
%have been evaluated for our intended testbed setup.
targeting the testbed of Section~\ref{testbed}.


%Assuming $N$ received samples, a set of observations can be expressed as
%\begin{equation}
%    \textbf{Y} = [y(t_0), y(t_1), \ldots, y(t_{N-1})].
%\end{equation}
\begin{comment}
The received signal $x(t)$ is transformed in the frequency domain via the FFT operation, to obtain $\mathbf{Y}$. Considering that one subcarrier represents a single snapshot, $\mathbf{Y}$ has dimensions $N_{\text{antennas}}\times N_{\text{subcarriers}}$. The covariance matrix of $\mathbf{Y}$ is %expressed as
\begin{equation}
    \textbf{R} = \text{E} [\mathbf{YY^T}].
    \label{cov matrix}
\end{equation}

The eigenvalue decomposition of the covariance matrix yields $M$ eigenvalues of $\textbf{R}$, $\lambda_1 \leq \lambda_2 \leq \ldots \leq \lambda_M$.

A log-likelihood function $L(n)$ is used to estimate the maximum likelihood of source number $n$, defined in \cite{Cheng} as
\begin{equation}
    L(n) = \frac{{(\lambda_{n+1} \lambda_{n+2} \ldots \lambda_{M})}^{\frac{1}{M-n}}}{\frac{1}{M-1}({\lambda_{n+1} + \lambda_{n+2} + \ldots + \lambda_{M})}}.
\end{equation}
\end{comment}
The AIC is often used %in the field of signal processing
to estimate the number of sources, $n$, in a mixture of signals. The AIC value deduced from $N$ samples is calculated for each possible $n$, subsequently selecting $n^*_{\text{AIC}}$, i.e., the candidate number of sources with the lowest AIC value, as the most appropriate estimator of the actual number, as described by
\begin{equation}
    n^*_{\text{AIC}} = \operatornamewithlimits{argmin}\limits_n\big[-2N(M-n) \log L(n) + 2n(2M-n)\big],
    \label{Akaike}
\end{equation}
where $L(n)$ is a log-likelihood function used to estimate the maximum likelihood of source number $n$, defined in \cite{Cheng} as
\begin{equation}
    L(n) = \frac{{(\lambda_{n+1} \lambda_{n+2} \ldots \lambda_{M})}^{\frac{1}{M-n}}}{\frac{1}{M-1}({\lambda_{n+1} + \lambda_{n+2} + \ldots + \lambda_{M})}}.
\end{equation}
The MDL principle is another widely used model selection criterion in statistical modeling and hypothesis testing. MDL calculates the coding length required to describe each candidate, taking into account both the parameters and the data. The candidate with the shortest coding length is selected as the most appropriate one, as described by
\begin{align}
     n^*_{\text{MDL}} = \operatornamewithlimits{argmin}_n\Big[{-}2N(M{-}n)&\log L(n) &
     \nonumber\\
     & +\frac{n}{2}(2M{-}n)\!\log N\Big ].
     \label{MDL}
\end{align}

The ECOD method estimates the number of sources using  the ratio of two consecutive eigenvalues, and  is described by 
\begin{equation}
    \operatorname{ECOD}(l) = \begin{cases}
    \frac{\lambda_l}{\lambda_{l-1} - 2\lambda_l}, &\text{$l>0$ and $\lambda_l \leq \frac{\lambda_{l-1}}{3}$} \\
    1, &\text{otherwise},
    \end{cases}
    \label{ECOD}
\end{equation}
where $l \in \{0, 1, \dots, M - 1\}$.
% Then, the corresponding minimum candidate is the appropriate to be selected as 
Then the number of sources is %estimated by~$n$, given by
\begin{equation}
    n^*_{\text{ECOD}} = \operatornamewithlimits{argmin}_l\big[\operatorname{ECOD}(l)\big].
    \label{ECOD2}
\end{equation}

%\begin{figure}
%\begin{tabular}{cc}
%        \includestandalone[width=.22\textwidth]{COE1}
% &
%    \includestandalone[width=.22\textwidth]{COE2} \\
%        \includestandalone[width=.22\textwidth]{COE3}
% &
%    \includestandalone[width=.22\textwidth]{COE4} \\
%\end{tabular}
%\caption{Comparison between Akaike, MDL and ECOD, when 1 MPC is present}
%\label{Ak v MDL v ECOD 1}
%\end{figure}

\begin{figure}
%\includegraphics{figs/COE9}
%\resizebox{.9\columnwidth}{!}
\input{figs/COE9}
%\includestandalone[width=.48\textwidth]{figs/COE9}
\caption{Comparison between Akaike, MDL and ECOD. The angle separation between the LOS and the MPC ranges from 5\degree{} to 20\degree.}
\label{Ak v MDL v ECOD 1}
\end{figure}

%\begin{figure}
%\input{figs/COE10}

%\includestandalone[width=\columnwidth]{figs/COE10}
%\caption{Comparison between Akaike, MDL and ECOD, for two MPCs. The angle separation between the LOS and the MPCs ranges from 5\degree{} to 20\degree.}
%\label{Ak v MDL v ECOD 2}
%\end{figure}

%\begin{figure}
%\begin{tabular}{cc}
%        \includestandalone[width=.22\textwidth]{COE5}
% &
%    \includestandalone[width=.22\textwidth]{COE6} \\
%        \includestandalone[width=.22\textwidth]{COE7}
% &
%    \includestandalone[width=.22\textwidth]{COE8} \\
%\end{tabular}
%\caption{Comparison between Akaike, MDL and ECOD, when 2 MPCs are present}
%\label{Ak v MDL v ECOD 2}
%\end{figure}

The three aforementioned criteria have been used in our model for channel-order estimation. A ``hit'' occurs when the estimated number of sources $n^*$ coincides with the actual scenario, otherwise it is considered a ``miss.'' Fig.~\ref{Ak v MDL v ECOD 1} compares the AIC, MDL and ECOD estimations of the number of sources, corresponding to a scenario of a LOS path set at 0\degree \space plus one MPC of half the LOS power. The angle in the legend entries of the figure denotes the discrepancy between the LOS path and the MPC. The figure depicts four different scenarios per criterion, regarding the discrepancy between the AoA of the LOS path and the MPC, ranging from 5\degree \space to 20\degree \space with a step of 5\degree. 
%The results can be distinguished in two different categories:
\ts{To perform Channel Order Estimation simulations with a 3-element ULA.}
\subsection{AoA Estimation Algorithms}
Three conventional Angle-of-Arrival algorithms have been studied and implemented: MUSIC \cite{MUSIC}, ESPRIT \cite{ESPRIT} and JADE ESPRIT \cite{2DESPRIT}. 
\begin{comment}
MUSIC is a super-resolution direction-finding algorithm, based on the eigenvalue decomposition of the received signal covariance matrix, defined in \eqref{cov matrix}. As per \eqref{cov matrix}, the covariance matrix has dimensions $M \times M$. This results in the MUSIC algorithm being able to detect up to $M -1$ sources. The eigenvectors corresponding to the $D$ larger eigenvalues of the covariance matrix span the signal subspace $\mathbf{U}_\text{s} = [\mathbf{v}_1,\dots,\mathbf{v}_D]$, whereas the remaining eigenvectors span the noise subspace $\mathbf{U}_\text{n} = [\mathbf{u}_{D+1},\dots,\mathbf{u}_{M-D}]$, where $D$ denotes the number of sources.

As the covariance matrix \textbf{R} is hermitian, all its eigenvectors are orthogonal to each other, meaning that the signal subspace is orthogonal to the noise subspace. The degree of orthogonality in the MUSIC algorithm is measured by
\begin{equation}
    \text{MUSIC}_{\text{Spectrum}} = \frac{1}{\mathbf{A^H U_n U_n^H A}},
\end{equation}
where $\mathbf{A}$ is the steering vector of received signal. 

ESPRIT divides the main element array into a set of subarrays. Assuming the subarrays $\mathbf{A_1}$ and $\mathbf{A_2}$, %these subarrays are related as 
it holds that
\begin{equation}
    \mathbf{A_2} =  \mathbf{A_1 \Xi},
    \label{rotation}
\end{equation}
where $\mathbf {\Xi}$ is a diagonal matrix whose main diagonal entries are $\xi_i = \exp\left({\frac{-2j \pi d \sin{\theta_i}}{\lambda}}\right)$, where $d$ is the antenna element spacing, $\theta_i$ denotes the Angle-of-Arrival $\theta$ at each antenna element  and $\lambda$ denotes the wavelength. Matrix $\mathbf{\Xi}$ applies a rotation to the matrix $\mathbf{A_1}$. Following \eqref{rotation}, ESPRIT exploits similar rotations in matrices formed by the eigenvectors of the covariance matrix of the measured data. 

After eigenvalue decomposition is performed and the signal subspace is separated from the noise subspace in a similar manner to the MUSIC algorithm, a matrix~$\mathbf{S}$ is formed,
\begin{equation}
\mathbf{S} = \mathbf{U_s}(:,1:D), \label{e:SU}
\end{equation}
where $\mathbf{U_s}$ is the matrix containing the eigenvectors. Notation in~\eqref{e:SU} denotes that $\mathbf{S}$ comprises the first $D$ columns of $\mathbf{U}$.

There exists a matrix $\mathbf{P}$ that contains rotational information such that the first set of eigenvectors yield the second set
\begin{equation}
    \mathbf{S_2} = \mathbf{S_1} \mathbf{P},
\end{equation}
which can be obtained via the Least Squares method, i.e.,
\begin{equation}
    \mathbf{P} = \frac{\mathbf{S}_1^* \mathbf{S}_2}{\mathbf{S}_1^* \mathbf{S}_1}.
\end{equation}

Lastly, the angle $\theta$ can be estimated in closed form, as
\begin{equation}
\theta  = \arcsin(\kappa),
\end{equation}
where
%\begin{equation}
 $   \kappa  = \frac{\phi_i}{2\pi d} $
 %\end{equation}
and~$\phi_i$ is the $i$-th phase angle of the total $K$ eigenvalues of~$\mathbf{P}$.

2D ESPRIT forms a Hankel matrix by stacking copies of CSI matrix $\mathbf{H}$. Similarly to 1D ESPRIT, the shift-invariant properties of the matrix are exposed. However, in this case, similar to the matrix $\mathbf{\Xi}$, a matrix $\mathbf{\Psi}$ is defined, whose main diagonal entries are $\psi_i = \exp\left({\frac{-2j \pi \tau_i}{L}}\right)$, where $L$ is the channel length measured in symbol periods. A data model given by
\begin{equation}
    \textbf{H} = \textbf{ABF}
    \label{model}
\end{equation}
is satisfied, where $\mathbf{A}$ is the Khatri-Rao product of the steering matrix with the delay matrix, $\mathbf{B}$ denotes the path attenuation and $\mathbf{F}$ is the DFT matrix with a Vandermonde structure. 

A set of selection matrices is also defined, in which $\xi_i$ and $\psi_i$ corresponding to the angles and delays, respectively, are estimated. The factor $\mathbf{F}$ in \eqref{model} ensures that a pairing between the angles and delays is satisfied. The correct pairing is carried out by a joint diagonalization procedure. To reduce complexity, all the computations can be kept in the real domain as described in \cite{UnitaryESPRIT}.
\end{comment}
MUSIC is a super-resolution direction-finding algorithm based on the eigenvalue decomposition of the covariance matrix \(\mathbf{R} \in \mathbb{C}^{M \times M}\). It detects up to \(M-1\) sources by decomposing \(\mathbf{R}\) into the signal subspace \(\mathbf{U}_s = [\mathbf{v}_1, \dots, \mathbf{v}_D]\) and the noise subspace \(\mathbf{U}_n = [\mathbf{u}_{D+1}, \dots, \mathbf{u}_M]\), where \(D\) is the number of sources. Since \(\mathbf{R}\) is Hermitian, these subspaces are orthogonal, and MUSIC exploits this via the spectrum:  
\begin{equation}
    \text{MUSIC}_{\text{Spectrum}} = \frac{1}{\mathbf{A}^H \mathbf{U}_n \mathbf{U}_n^H \mathbf{A}}
\end{equation}
where \(\mathbf{A}\) is the steering vector.


ESPRIT divides the main element array into subarrays \(\mathbf{A_1}\) and \(\mathbf{A_2}\), related as  
\begin{equation}
    \mathbf{A_2} =  \mathbf{A_1 \Xi},
    \label{rotation}
\end{equation}
where \(\mathbf{\Xi}\) is a diagonal matrix with entries  
\[
\xi_i = \exp\left(\frac{-2j \pi d \sin{\theta_i}}{\lambda}\right),
\]  
where \(d\) is the antenna spacing, \(\theta_i\) the Angle-of-Arrival, and \(\lambda\) the wavelength. ESPRIT exploits this rotational structure in the signal subspace \(\mathbf{U_s}\), forming  
\begin{equation}
\mathbf{S} = \mathbf{U_s}(:,1:D), \label{e:SU}
\end{equation}
where \(\mathbf{S}\) contains the first \(D\) columns of \(\mathbf{U_s}\). A matrix \(\mathbf{P}\) relates the subspaces:  
\begin{equation}
    \mathbf{S_2} = \mathbf{S_1} \mathbf{P},
\end{equation}
estimated via Least Squares:  
\begin{equation}
    \mathbf{P} = \frac{\mathbf{S}_1^* \mathbf{S}_2}{\mathbf{S}_1^* \mathbf{S}_1}.
\end{equation}
The angle \(\theta\) is then estimated as  
\begin{equation}
\theta  = \arcsin(\kappa),
\end{equation}
where  
\[
\kappa = \frac{\phi_i}{2\pi d}
\]  
and \(\phi_i\) is the \(i\)-th phase of the \(K\) eigenvalues of \(\mathbf{P}\).


2D ESPRIT forms a Hankel matrix by stacking copies of the CSI matrix \(\mathbf{H}\), exposing its shift-invariant structure. Similar to the 1D case, a diagonal matrix \(\mathbf{\Psi}\) with entries 
\[
\psi_i = \exp\left(\frac{-2j \pi \tau_i}{L}\right),
\]
is defined, where \(L\) is the channel length (in symbol periods). The data model is
\begin{equation}
    \mathbf{H} = \mathbf{A B F},
    \label{model}
\end{equation}
with \(\mathbf{A}\) as the Khatri-Rao product of the steering and delay matrices, \(\mathbf{B}\) representing path attenuation, and \(\mathbf{F}\) a DFT matrix with Vandermonde structure.  
Selection matrices extract \(\xi_i\) and \(\psi_i\) (for angles and delays, respectively), and \(\mathbf{F}\) in \eqref{model} ensures proper angle-delay pairing via joint diagonalization. For reduced complexity, computations can be performed in the real domain as in~\cite{UnitaryESPRIT}.
